MVDiffusion++: A Dense High-resolution Multi-view Diffusion Model for Single or Sparse-view 3D Object Reconstruction

This paper presents a neural architecture MVDiffusion++ for 3D object reconstruction that synthesizes dense and high-resolution views of an object given one or a few images without camera poses. MVDiffusion++ achieves superior flexibility and scalability with two surprisingly simple ideas: 1) A ``pose-free architecture'' where standard self-attention among 2D latent features learns 3D consistency across an arbitrary number of conditional and generation views without explicitly using camera pose information; and 2) A ``view dropout strategy'' that discards a substantial number of output views during training, which reduces the training-time memory footprint and enables dense and high-resolution view synthesis at test time. We use the Objaverse for training and the Google Scanned Objects for evaluation with standard novel view synthesis and 3D reconstruction metrics, where MVDiffusion++ significantly outperforms the current state of the arts. We also demonstrate a text-to-3D application example by combining MVDiffusion++ with a text-to-image generative model. The project page is at https://mvdiffusion-plusplus.github.io.

==> figures/sparse_mesh_qualitative.tex <==
\begin{figure}
\centering
\includegraphics[width=\textwidth]{assets/multi_view_mesh.pdf}
\caption{Qualitative comparison between NeuS~\cite{wang2021neus} with G.T. poses and \ourmethod~in sparse-view 3D reconstruction. }
\label{fig:sparse-mesh}
\end{figure}

==> sections/0-abstract-eccv.tex <==
\begin{abstract}
This paper presents a neural architecture {\ourmethod}~for 3D object reconstruction that synthesizes dense and high-resolution views of an object given one or a few images without camera poses. \ourmethod~achieves superior flexibility and scalability with two surprisingly simple ideas: 1) A ``pose-free architecture'' where standard self-attention among 2D latent features learns 3D consistency across an arbitrary number of conditional and generation views without explicitly using camera pose information; and 2) A ``view dropout strategy'' that discards a substantial number of output views during training, which reduces the training-time memory footprint and enables dense and high-resolution view synthesis at test time. We use the Objaverse for training and the Google Scanned Objects for evaluation with standard novel view synthesis and 3D reconstruction metrics, where \ourmethod~significantly outperforms the current state of the arts. We also demonstrate a text-to-3D application example by combining {\ourmethod} with a text-to-image generative model.
%extensive qualitative results with real-world images.


%Extensive evaluations demonstrate that \ourmethod~excels in novel view synthesis and generalizes to in-the-wild objects, and enables high-quality single or sparse-view object reconstructions. 
\end{abstract}


==> sections/3-preliminary-eccv.tex <==
\section{Preliminary: Multi-view latent diffusion models}
\label{sec:preliminary}

MVDiffusion~\cite{tang2023mvdiffusion} is a multi-view latent diffusion model~\cite{tang2023mvdiffusion,shi2023mvdream,liu2023syncdreamer,shi2023zero123++}, generating multiple images given a text or an image, when pixel-wise correspondences are available across views.
MVDiffusion is the foundation of the proposed approach, where the section reviews its architecture and introduces notations (See \autoref{fig:equations}).

%nd reviews MVDiffusion~\cite{tang2023mvdiffusion}, a foundation of the proposed approach (See \autoref{fig:mvdiffusion_equations}).
% consists of multiple branches of a standard image latent diffusion model, particularly Stable Diffusion (SD)~\cite{rombach2022high}. 
%our prior work and the foundation of the proposed method.
%
\begin{comment}
\mypara{Latent diffusion models}
Latent Diffusion Model (LDM)~\cite{rombach2022StableDiffusion} has been a core machinery in the recent explosion of content generation techniques. 
LDM consists of a variational autoencoder (VAE)~\cite{kingma2013vae} with encoder $\encoder$ and decoder $\decoder$, a denoising network $\model$, and a condition encoder $\conditioner$. 
Raw images $\img \in \mathbb{R}^{\hpixel \times \wpixel \times \cpixel}$ are mapped to a compressed latent space by $\latent=\encoder(\img)$, $\latent \in \mathbb{R}^{\hlatent \times \wlatent \times \clatent}$, and the latents are converted back to image by $\imgrec = \decoder(\latent)$. 
The training objective is defined as
\begin{align}
\lsimpleldm := \expec_{ \encoder(\img), \cond, \bepsilon \sim \mathcal{N}(0, 1), t }\Big[ \Vert \bepsilon - \model(\latent_{t},t, \conditioner(\cond)) \Vert_{2}^{2}\Big] 
\label{eq:cond_ldm_loss}
\end{align}
The denoising network $\model$ is a UNet-like architecture with several blocks. Each block consists of the following layers.
\begin{align}
    F^l_S&=\text{SA}(F^{l}) \\
    F^l_C&=\text{CA}(F^l_S, \text{CLIP}(I)) \\
    F^{l+1}&=\text{Conv}(F^l_C, t),
\end{align}
where $\text{SA}$ is the self attention layer, $\text{CA}$ is the cross attention layer, $\text{Conv}$ is several convolution layers, $\text{CLIP}$ is the CLIP image encoder and $I$ is the raw image.
% where $t$ is uniformly sampled from $1$ to $T$ and $\latent_{t}$ is the noisy latent at time step $t$. The denoising network $\model$ is a UNet~\cite{dhariwal2021guided-diffusion} augmented with cross-attention mechanisms to incorporate the time embedding and the optional condition encoding $\conditioner(\cond)$. 
% At sampling time, the reverse process generates samples in the latent space with advanced samplers~\cite{song2020ddim,karras2022edm}, and the VAE decoder outputs final images with a single forward pass. 
\end{comment}
%
%\mypara{Multi-view latent diffusion models}
%MVDiffusion extends a latent diffusion model~\cite{rombach2022StableDiffusion} to generate multiview images,
%Recent 3D modeling works have fine-tuned LDM to generate consistent multi-view images,
 
For generating eight perspective views forming a panorama, 
%MVDiffusion architecture consists of 
eight latent diffusion models (LDM) denoise eight noisy latent images $\{\latent_1(t), \latent_2(t), \cdots \latent_8(t) \}$ simultaneously.
%$\latent_i(t)$ is the noisy latent of the $i$-th image at timestep $t$. 
%$T$ is the largest timestep.
%
%total number of timesteps.
%of the diffusion model.  
A UNet is the core of a LDM model, 
%At a denoising step $t$, a CNN initializes the UNet input 
%$t$ is a timestep.
consisting of a sequence of blocks through the four levels of the feature pyramid.


Let $U^i_b$ denote the feature image of $i$-th image at $b$-th block. A CNN initializes an input $U^0_i$ from $\latent_i(t)$ at the first block.
%each denoising step $t$.
%
Each UNet block has four network modules.
The first is a novel correspondence-aware attention (CAA), enforcing consistency across views with visual overlaps: The left/right neighboring images ($U^b_{i-1}, U^b_{i+1}$) for panorama.
%e case of panorama. 
%To maintain view consistency, MVDiffusion incorporates
%With an abuse of the superscript, we denote the features of $i$-th image at the $b$-th UNet block as $U_i^b$.
The remaining three modules are from the original:
%In SD models, the UNet block consists of three network modules:
1) Self-attention (SA) layers; 2) Cross-attention (CA) layers from the condition with the CLIP embedding; and 3) CNN layers with the pixel-wise concatenation of a positional encoding of time $\tau(t)$. At test time, a standard DDPM sampler~\cite{ho2020denoising} updates all noisy latents with the predicted noise from the last CNN layer.
%MVDiffusion adds novel correspondence-aware attention layers (CAA) to ensure view consistency, which is a form of cross attention from other views with visual overlaps (e.g., $(N^b_{i-1}, N^b_{i+1}$) for this panorama case).
%layer $l$ of the UNet block as $U_i^l$.
%, a form of CA layers from views with visual overlaps.
%, $(N^b_{i-1}, N^b_{i+1})$ in the panorama scenario.
%Omitting the condition for notation simplicity, t
The training objective is defined as follows by omitting the conditions for notation simplicity, where $\bepsilon^i$ is a Gaussian and $\model$ denotes the UNet output.
\begin{align}
\lsimplemv
:= \expec_{\left\{ \latent_i(0) \right\}_{i=1}^N, \left\{\bepsilon^i \sim \mathcal{N}(0, I)\right\}_{i=1}^N, t} \Big[ \sum_{i=1}^N \Vert \bepsilon^i - \model^i(\left\{ \latent_i(t) \right\}, \tau(t)) \Vert_{2}^{2}\Big].
\label{eq:cond_mvldm_loss}
\end{align}



%noisy latent of the $i_{\text{th}}$ image
%Two fundamental extensions are made to adapt a pre-trained LDM to multiple images: 1) the forward process injects noises into all the image patients, 2) the denoising network is modified to take all the noisy latent and denoise them simultaneously, and 3) A correspondence-aware attention mechanism (CAA) to build connection across all the views. The UNet block architecture is modified to the following:
%

\begin{comment} 
\begin{tabularx}{\columnwidth}{|C|} \hline
    $\forall{i}\ N^{l}_i \hspace{0.34cm} \leftarrow \mathbf{CAA}(\{N^l_{i-1},N^l_{i+1}\}, N^l_i)$ \\   $\forall{i}\ N^l_i \hspace{0.34cm} \leftarrow \mathbf{SA}(N^l_i)$ \\
    $\forall{i}\ N^l_i \hspace{0.34cm} \leftarrow \mathbf{CA}(\mathbf{CLIP}(I_{\text{mage}} \ \text{or} \ T_{\text{ext}}), N^l_i)$ \\
    $\forall{i}\ N^{l}_i \hspace{0.34cm} \leftarrow \mathbf{CNN}(\left[N^l_i, \gamma(t)\right])$ \\
 \hline
\end{tabularx}

\noindent
\begin{tabularx}{\columnwidth}{|l||l|l|} \cline{1-3}
& 
\multicolumn{1}{l|}{\text{Generation view}} & \multicolumn{1}{l|}{\text{Conditional view}} \\ \cline{1-3} 
    $\forall{i}\ N^l_i \hspace{0.34cm} \leftarrow$ &
    $\orange{\left[N^l_i, \mathbf{MVAE}(\left[I_i, M_i\right]), \mathfrak{M}_{pos}\right]}$ &
    $\orange{\left[N^l_i, \mathbf{MVAE}(\left[\mathfrak{I}_{white}, \mathfrak{M}_{pos} \right]), \mathfrak{M}_{neg}\right]}$ \\
    $\orange{\{N^l_*\}} \hspace{0.39cm}  \leftarrow$ & 
    $\orange{\mathbf{SA}(\{N^l_*\})}$ &
    $\orange{\mathbf{SA}(\{N^l_*\})}$ \\
    $\forall{i}\ N^l_i \hspace{0.34cm} \leftarrow$ & 
    $\mathbf{CA}(\mathbf{CLIP}(\orange{I_i}), N^l_i)$ & 
    $\mathbf{CA}(\mathbf{CLIP}(\orange{\mathfrak{W}_{hite}}), N^l_i)$  \\ 
    $\forall{i}\ N^{l}_i \hspace{0.34cm} \leftarrow$ &
    $\mathbf{CNN}(\left[N^l_i, \gamma(t) \orange{+ \gamma(G_?)}\right])$ &
    $\mathbf{CNN}(\left[N^l_i, \gamma(t) \orange{+ \gamma(C_?)}\right])$ \\ 
    \cline{1-3}
\end{tabularx}
\end{comment}


\begin{comment}
% 
%    $\forall{i}\ \ F_i \leftarrow
%    \left\{\begin{array}{ll}
%        \text{Concat}(F_i, \text{MVAE}(I_i), \mathfrak{B}_{pos}) & \ \  \text{(if generation view)} \\
%        \text{Concat}(F_i, \text{MVAE}(\mathfrak{I}_{white}), \mathfrak{B}_{neg}) & \ \ \text{(if conditional view)}  
%    \end{array} \right.$ \\

\begin{tabularx}{\columnwidth}{|C|C|} \hline
    \forall{i}\ \ F_i \leftarrow \text{SA}(F_i) 
    & \\
    \forall{i}\ \ F_i \leftarrow \text{CA}(\text{CLIP}(Text), F_i)
    & \\
    \forall{i}\ \ F_i \leftarrow \text{Conv}(\text{Concat}(F_i, t))
    & \\
    \forall{i}\ \ F_i \leftarrow \text{CAA}(\{F_{i-1},F_{i+1}\}, F_i)                 
    & \\ \hline
\end{tabularx}

\begin{tabularx}{\columnwidth}{|C|C|} \hline
    \forall{i}\ \ F^i_{*,*} \leftarrow \text{SA}(F^i_{*,*}) 
    & \\
    \forall{i}\ \ F^i_{*,*} \leftarrow \text{CA}(\text{CLIP}(Text), F^i_{*,*})
    & \\
    \forall{i,x,y}\ \ F^i_{x,y} \leftarrow \left[F^i_{x,y}, t \right]
    & \\
    \forall{i}\ \ F^i_{*,*} \leftarrow \text{Conv}(F^i_{*,*})
    & \\
    \forall{i}\ \ F^i_{*,*} \leftarrow \text{CAA}(\{F^{i-1}_{*,*},F^{i+1}_{*,*}\}, F^i_{*,*})                 
    & \\ \hline
\end{tabularx}


\begin{align}
\end{align}
%
\begin{align}
    F^l_S&=\text{SA}(F^{l}) \\
    F^l_C&=\text{CA}(F^l_S, \text{CLIP}(I)) \\
    F^l_{O}&=\text{Conv}(F^l_C, t) \\
    F^{l+1}&=CAA(F^l_{O}),
\end{align}
%
%\begin{align}
%    F^l_S&=\text{SA}(F^{l}) \\
%    F^l_C&=\text{CA}(F^l_S, \text{CLIP}(I)) \\
%    F^l_{O}&=\text{Conv}(F^l_C, t) \\
%    F^{l+1}&=CAA(F^l_{O}),
%\end{align}
%The general training objective of the multi-view LDM can be defined as
\yasu{We may not need to define a loss function here, unless this helps the main section 4, but we do not seem to talk about loss in the main section now, and I cannot tell if we need this.}
\end{comment}
%
%\yasu{We say "Two fundamental extensions" but there are 3. The 4 equations here and notations are not good, but this must be designed with the main section 4 to highlight the differences from LDM, mvdiffusion and mvdiffusion++, and we will come back. The key design differences must be immediately clear when looking at notations, which are currently not.}
%
\begin{comment}
Previous works mainly differ in the designs of the multi-view denoising network $\model$, including how the conditions are incorporated and how the information between multiple generated views is synchronized. The essential contributions of \ourmethod~are two-folded: 1) an inpainting-style formulation for $\model$, which flexibly takes any number of pose-free condition images and generates multi-view images, and 2) a simple yet effective training strategy, view dropout, which enables the model to generate dense multi-view images at higher resolutions. 
\end{comment}




==> sections/4-method-eccv.tex <==
\section{\ourmethod}
%
%over the current state-of-the-art (MVDiffusion~\cite{tang2023mvdiffusion}, SyncDreamer~\cite{liu2023syncdreamer}, and Wonder3D~\cite{long2023wonder3d}) 
%pushing the frontier of multi-view diffusion models in the scalability and flexibility over the current state-of-the-art such as MVDiffusion~\cite{tang2023mvdiffusion}, SyncDreamer~\cite{liu2023syncdreamer}, and Wonder3D~\cite{long2023wonder3d}.
% complete 3D modeling requires dense and high-resolution 


\ourmethod~pushes the frontier of multi-view diffusion models for 3D modeling in their \textit{flexibility} and \textit{scalability} by generating dense and higher-resolution images given an arbitrary number of un-posed condition views.
%
With the prevalence of Transformer models~\cite{vaswani2017transformer}, high-fidelity 3D modeling would require large-scale attention over dense and high-resolution image features, potentially with volumetric ones. Furthermore, 3D consistency learning is at the heart of the task, which would usually require precise image projection models and/or camera parameters. %with the attention mechanism.
%
%a key advantage over the existing multi-view diffusion models such as MVDiffusion~\cite{tang2023mvdiffusion}, SyncDreamer~\cite{liu2023syncdreamer}, and Wonder3D~\cite{long2023wonder3d}.
%
%This flexibility poses major technical challenges, as 3D consistency learning is at the heart of the task, which usually involves image projection models and camera parameters.
%, image projection models, and/or epipolar geometry.
%
Our surprising discovery is that self-attention among 2D latent image features is all we need for 3D learning without projection models or camera parameters,
and a simple training strategy would further achieve dense and high-resolution multi-view image generation.
%Note that we do not pass camera parameters of output views at all. 
%
%Furthermore, camera poses of the input views are unknown and change per sample. 
%\ourmethod~ without requiring pixel-wise correspondences across output views. While being a surprisingly simple extension of MVDiffusion, the proposed architecture effectively generates high-quality images that are consistent in 3D and readily available for 3D reconstruction.
%
%These high-fidelity generated images provide rich details of an object from almost all perspectives, making them easily used for 3D reconstruction. 
%
% with NeRF~\cite{mildenhall2020nerf}, NeuS~\cite{wang2021neus}, or their variants. 
% The core of \ourmethod~is an inpainting-style multi-branch and multi-view diffusion model, initialized from latent Diffusion inpainting model~\cite{rombach2022high}. 
% Figure~\ref{fig:overview} shows an overview of the method, and 
The section defines the task (i.e., input condition and output target images), then explains the two key ideas: 1) pose-free multi-view conditional diffusion model for flexibility and 2) view dropout training strategy for scalability.
\S\ref{sec:details} provides the remaining system details.
%for reproducibility.


%
%This section is organized as follows: \S\ref{subsec:camera} describes the camera configurations of the conditional and generated images. \S\ref{subsec:vae-ft} introduces the VAE fine-tuning for simultaneous foreground mask modeling and less encoding information loss. \S\ref{subsec:dm} and \S\ref{subsec:view-drop} demonstrate our key innovations, the pose-free multi-view conditional diffusion model and the view dropout training strategy, respectively. Finally, \S\ref{subsec:detail} discusses the training details and how we export meshes from the generated images.

\subsection{Task: Input condition images and output target images}
\label{subsec:camera}

%\input{figures/camera_configuration}
\input{figures/equations}
%
%Objaverse dataset~\cite{deitke2023objaverse} 
%Google scanned object dataset for evaluation

\input{figures/method}

%
%The specifics of the task settings may vary slightly between datasets used for training and testing, which are elaborated on in \S\ref{sec:details}. This section emphasizes the shared task settings.
%The task settings slightly differ depending on the datasets during training and testing, whose details are referred to \S\ref{sec:details}. This section focuses on the common task settings.

The generation target is a set of dense (32) and high-resolution (512$\times$512) images, positioned at uniform 2D grid points on a sphere. Specifically, there are eight azimuth angles (every 45$^\circ$) and four elevation angles (every 30$^\circ$ in the range $[-30^\circ, 60^\circ]$). 
Camera up-vectors are aligned with gravity, and their optical axes pass through the sphere center.
%
Our input condition is one or a few images without camera poses, where visual overlaps are too minimal or possibly none for Structure from Motion algorithms to work reliably. The number of condition images is up to a pre-determined number, which is $10$ in our experiments but can easily change. The input image resolution is 512$\times$512. The horizontal and vertical field-of-view of both the input and output views is 60$^\circ$.


%Camera centers are positioned on a sphere with a radius $1.5m$ 


We use synthetic rendered images from 3D object databases for training and evaluations.
 %
The task settings vary slightly between datasets, with details provided in \S\ref{sec:details}.
%We use 3D object databases to synthesize images.
%condition and target images for experiments.
%\S\ref{sec:details} provides the full details of the processes, while 
Here, we explain one preprocessing step that removes ambiguity in the training task.
%the rest of the section explains one preprocessing step,
%of the processes, while the rest of the section explains one pre-processing step.
%which removes an ambiguity in our task.
3D object databases such as Objaverse~\cite{deitke2023objaverse} and Google Scanned Object~\cite{downs2022gso} align the Z-axis with the object up-vectors. 
%In real scenarios, gravity is available from phone sensors such as IMU. Therefore, we assume that the image Y-axis is aligned with gravity.
However, the azimuth of the ground-truth object pose is ambiguous without 
%this leaves one ambiguity in our task. W
camera poses of the condition images.
%defined up to a 1D rotational around azimuth. 
Therefore, we rotate the output views to align the azimuth of the first condition and the first output image.
%to make the training task feasible.
%so that the azimuth angle of the first condition image becomes 0$^\circ$.


%The above task is ill-posed due to the rotational ambiguity along an azimuth in the output images: 




%whose processes slightly differ at training and testing.

%he elevations are 60$^\circ$, 30$^\circ$, 0$^\circ$, and -30$^\circ$ in the default object coordinate system of Objaverse where all objects are upright and z-axis aligned.
%

%During training, given an object 3D model from Objaverse dataset~\cite{deitke2023objaverse}, we use the object coordinate frame to calculate 32 generation views


\subsection{Pose-free multi-view conditional diffusion model}
\label{subsec:dm}

%This section explains our ``pose-free'' mulit-view diffusion models, while the next section explains the view-dropout training strategy, which is crucial for training our architecture.


%we allow the model to take an arbitrary number of input views (1-10), making the model suitable for both single and sparse-view conditioning; 2) the model does not require camera poses, refraining us from the challenging pose estimation process when input images are sparse and have limited overlaps.

%We employ the general framework of multi-view LDM as described in \S\ref{sec:preliminary} and focus on proposing a more flexible architecture for the multi-view denoising network $\model$. Compared to previous multi-view diffusion models such as MVDiffusion~\cite{tang2023mvdiffusion}, SyncDreamer~\cite{liu2023syncdreamer}, or Wonder3D~\cite{long2023wonder3d}, etc, 

%Inspired by the image-to-panorama variant of MVDiffusion~\cite{tang2023mvdiffusion}, our denoising network $\model$ is formulated as an inpainting-style model and initialized from latent Diffusion's inpainting model.
\ourmethod~is a multi-view latent diffusion model as defined in \S\ref{sec:preliminary}, comprising of a \textit{condition branch} for single or sparse-view input images and a \textit{generation branch} for output images (See \autoref{fig:equations} and \autoref{fig:overview}). Note that the condition branch shares the same architecture and is tasked to generate the condition images that are also given as guidance (i.e., a trivial task).


\mypara{Diffusion process}
The forward diffusion process is the same as MVDiffusion, except for the image resolution and the pre-trained VAE. Concretely, it 1) converts all $512\times 512\times 3$ input/output image ($I_i$) with foreground masks to $64\times 64\times 4$ latent images ($Z_i$) by a fine-tuned latent diffusion VAE (denoted as MVAE, see \S\ref{sec:details} for the fine-tuning process); and 2) adds a Gaussian noise with a linear schedule, as suggested by zero-123++~\cite{shi2023zero123++} to each feature of $Z_i$.


\mypara{Denoising process}
The denoising process is highlighted in \autoref{fig:equations}, where a latent diffusion UNet with a few modifications processes a noisy latent $Z_i(t)$ at each denoising step $t$. The UNet consists of $9$ blocks of network modules over the four levels of feature pyramids on either side of the encoder/decoder. The details are explained as follows.
% \yasu{weak start of an important section? come back here for re-editing}


\myparapara{[At first block]}
The UNet feature $U^0_i$ at the first block is initialized with the concatenation of 1) the noisy latents $Z_i$; 2) a constant binary mask of either 1 or 0, denoted by $\mathfrak{M}_{pos}$ or $\mathfrak{M}_{neg}$ to indicate the branch type (condition or generation); and 3) the condition latents ($\text{MVAE}(I_i, M_i)$) where we use the conditonal VAE from latent diffusion to encode the condition image ($I_i$) with its segmentation mask ($M_i$). 
%
Note that this concatenation has $9=(4+4+1)$ channels, and a $1\times1$ final convolution layer reduces the channel dimension to $4$.
%
For a generation branch, we pass a white image 
as $I_i$ and a binary image of 1 (i.e., $\mathfrak{M}_{pos}$) as $M_i$. 
For Objaverse and Google Scaned Object datasets, we use the masks provided by the datasets. Otherwise, we run segmentation to generate the masks.
% For images from the Internet, we use a third-party segmentation software clipdrop~\cite{clipdrop}.




\myparapara{[For each block]}
Three network modules process the input: 1) Global self-attention mechanism among the UNet features across all the images, learning 3D consistency; 2) Cross-attention mechanism, injecting the CLIP embedding of the condition images to all the other images through the CLIP embedding; and 3) CNN layers, process per-image features while injecting the timestep frequency encoding $\tau(t)$ and the learnable embedding of an image index $V_i$.
%, all UNet copies from the two branches are interconnected by self-attention mechanisms among the patch-level latent tokens.
%
For the self-attention module, we copy the network architecture and model weights 
% from the standard stable diffusion model~\cite{blattmann2023stablevideodm}, 
and apply it across all the views. This module is inspired by MVDream~\cite{shi2023mvdream}, while the key differences in our work are 1) Scalability deployment via the view-drop training strategy in \S\ref{subsec:view-drop}; and 2) Handling of multiple condition images without camera poses via the network design.
%blocks are from the stable diffusion models~\cite{rombach2022StableDiffusion}.
%original latent diffusion models~\cite{rombach2022StableDiffusion} are reused to learn multi-view 3D consistencies between all conditional and generated images. 
%
%his global multi-view attention is expected to learn three-level relations to enforce multi-view consistency: 1) between conditional images, 2) from conditional images to generation images, and 3) between generation images.
%
%The view embedding
%
%We use learnable view embeddings to distinguish different images. The condition branch has two learnable view embeddings: $\tau(V_1^C)$ is assigned to the reference view $C_{r}$, and $\tau(V_2^C)$ is assigned to all other conditional views. Each fixed viewpoint 
$42=(32+10)$ learnable embedding vectors $\{V_{i}\}$ are trained for 32 generation and 10 condition images, each of which is multiplied with a zero-initialized trainable scale $s$ to avoid model disruption at initailization.
%
%As shown by Figure~\ref{fig:overview}, the view embeddings are added to the timestep embedding $\tau(t)$ and injected into each UNet copy. 
%We multiply the view embeddings by a zero-initialized trainable scale $\alpha$ to avoid model disruption at initialization. 

\myparapara{[At last block]} The output of the last UNet block yields the noise estimation, and a standard DDPM sampler~\cite{ho2020denoising} takes it to produce the noisy latent of the next timestep $Z_i(t-1)$ for each sampling step. The loss function is the same as MVDiffusion. Note that the model is first trained with $\epsilon$-prediction and then with v-prediction (See \S\ref{sec:details}), where \autoref{eq:cond_mvldm_loss} is the loss function for the $\epsilon$-prediction model. The velocity~\cite{salimans2022progressive-v-pred}, $\bv^i(t) = \alpha_t \bepsilon^i - \gamma_t \latent_i(0) $,  becomes the prediction target for the v-prediction model, while $\alpha_t$ and $\gamma_t$ are predefined angular parameters.


%at fixed viewpoints with respect to the reference view.  
%two branches: a \textit{conditional branch} to digest single or sparse-view inputs, and a \textit{generation branch} to synthesize consistent dense multi-view images at fixed viewpoints with respect to the reference view.  
%Following MVDiffusion~\cite{tang2023mvdiffusion}, a variant of a standard image latent diffusion model, in particular, stable diffusion UNet generates each image in each branch.


\subsection{View dropout training strategy}
\label{subsec:view-drop}
\ourmethod~training would face a scalability challenge.
%Training the proposed \ourmethod~architecture would face two challenges.
%
%Training a global self-attention module over $42(=32+10)$ copies of UNet 
$42(=32+10)$ copies of UNet features yield more than 130k tokens, where the global self-attention mechanism becomes infeasible even with the latest memory efficient transformers for large language models~\cite{dao2022flashattention,dao2023flashattention2}.
%
%\myparapara{Computational feasibility} 
%Global self-attention mechanism over $42(=32+10)$ copies of UNet features would lead to 130k tokens, whose training is infeasible even with the latest memory efficient transformers for large language models~\cite{dao2022flashattention,dao2023flashattention2}.
% High-fidelity 3D object reconstruction could need hundreds of higher-resolution images, requiring a few orders of magnitude more tokens.
%
%Second, dense images lead to excess redundant signals, where generative model research on large images~\cite{chen2023importance_noise} or videos~\cite{blattmann2023stablevideodm} suggest that diffusion models suffer from the reduction of signal-to-noise ratio. 
%
%Our early experiments indeed revealed that the generation quality degrades even 
%
%showed that too-dense training views could hurt the generation quality even when we shift the noise schedule towards higher noise values following the suggestions of previous works~\cite{xxxxx}. \yasu{which paper said this?}
%
%The dense training views can lead to excess redundant signals, making it hard for the diffusion process to decrease the signal-to-noise ratio (SNR), which is similar to the case of training diffusion models for large images~\cite{chen2023importance_noise} or videos~\cite{blattmann2023stablevideodm}. Our early experiments showed that too-dense training views could hurt the generation quality even when we shift the noise schedule towards higher noise values following the suggestions of previous works.
%
%progress in memory-efficient transformers for large language models~\cite{dao2022flashattention,dao2023flashattention2}, state-of-the-art attention techniques can already afford a large number of tokens. 
%
%Considering images with resolution 512$\times$512, each image latent has size 64$\times$64. 32 generated images and 1-10 conditional images will lead to more than 130K tokens for the multi-view self-attention in the first and last UNet block. Handling even a million tokens has become possible with advanced memory-efficient attention, but since the training of multi-view diffusion models usually requires much more memory than inference, the training process of 42 high-resolution images is not feasible even with the most powerful GPU in the world. 
%
%\myparapara{Information redundancy} 
%
We propose a simple yet surprisingly effective \textit{view dropout} training strategy, which
%a view-level uniform dropout that 
completely discards a set of views across all layers during training. Specifically, we randomly drop 24 out of 32 views for each object at each training iteration, significantly reducing memory consumption at training.
%which significantly reduces the training cost.
At test time, we run the entire architecture and generate 32 views.
%, which works surprisingly well.
%\yasu{A bit shallow. we want some intelligent sentence to claim why this work...}

%the model is able to generate an arbitrary subset of the 32 views. Furthermore, due to the information redundancy issue discussed above, training with our view dropout leads to better generation quality than training with a full 32 views. We provide a tentative theoretical analysis in the \supp.


%We found even a large drop rate can work well in practice. 


%\dilin{Assume V the feature tokens, which is a composition of underlying features from GT inputs and noise, denoted as M and N, respectively. The key observation is that softmax will reduce the noise level proportionally to the square of the number of tokens. To illustrate this, let's denote W as the output of the softmax, and W is self-normalized. var(W'N) = W'var(N)W. In the case where W is uniform, this would exactly represent the quadratic relationship with respect to the number of tokens.}



%The dense training views can lead to excess redundant signals, making it hard for the diffusion process to decrease the signal-to-noise ratio (SNR), which is similar to the case of training diffusion models for large images~\cite{chen2023importance_noise} or videos~\cite{blattmann2023stablevideodm}. Our early experiments showed that too-dense training views could hurt the generation quality even when we shift the noise schedule towards higher noise values following the suggestions of previous works.





\begin{comment}
The huge computation cost used to be a core limitation for the above multi-view global attention, but thanks to the progress in memory-efficient transformers for large language models~\cite{dao2022flashattention,dao2023flashattention2}, state-of-the-art attention techniques can already afford a large number of tokens. Using the attention implementations in Diffusers~\cite{diffusers} together with our view dropout training strategy (described in \S\ref{subsec:view-drop}), our multi-view conditional diffusion model manages to take up to 10 conditional images and generate 32 dense images, all at resolution 512$\times$512, providing broader coverage and richer details for the objects. 



Based on the camera configuration and the model architecture described in \S\ref{subsec:camera}  and \S\ref{subsec:dm}, \ourmethod~needs to process up to 42 UNet copies (i.e., 10 conditional ones and 32 generated ones) in a single forward pass with global multi-view self-attention. Empirically, we find that training the model with this amount of high-resolution images presents two challenges:

\begin{enumerate}
[label={ {(\arabic*)}},leftmargin=*,topsep=0.5ex,itemsep=-0.5ex,partopsep=0.75ex,parsep=0.75ex,partopsep=0pt,wide, labelwidth=!,labelindent=0pt]

\item {\bf Computational feasibility.} Considering images with resolution 512$\times$512, each image latent has size 64$\times$64. 32 generated images and 1-10 conditional images will lead to more than 130K tokens for the multi-view self-attention in the first and last UNet block. Handling even a million tokens has become possible with advanced memory-efficient attention, but since the training of multi-view diffusion models usually requires much more memory than inference, the training process of 42 high-resolution images is not feasible even with the most powerful GPU in the world. 

\item {\bf Information redundancy.} The dense training views can lead to excess redundant signals, making it hard for the diffusion process to decrease the signal-to-noise ratio (SNR), which is similar to the case of training diffusion models for large images~\cite{chen2023importance_noise} or videos~\cite{blattmann2023stablevideodm}. Our early experiments showed that too-dense training views could hurt the generation quality even when we shift the noise schedule towards higher noise values following the suggestions of previous works.
\end{enumerate}

\end{comment}






% To make this more manageable and efficient, we implement a strategy of dropping a considerable number of generation views during training. Specifically, for each training object, we randomly select $N$ images from a set of 32 pre-rendered images. These selected images, along with the conditional images, are then used to train each UNet unit. Importantly, 3D self-attention is applied across all these sampled views. During the inference phase, our model demonstrates the capability to generate an arbitrary number of views given the corresponding camera embeddings, with 3D self-attention applied to all these generated views. This method of view dropout is akin to the commonly used attention dropout technique in network training, serving as an effective regularization method. Empirically, we have found that even a small number of views (setting $N=8$) can yield satisfactory performance.


\begin{comment}

\dilin{
Very very brief explanation of view drop: 
Assuming $n$ noisy views $\{v'_i\}_{i=1}^n$ with each view $v'_i = v_i + \epsilon_i$, where $v_i$ is the underlying real information and $\epsilon_i$ is the noise.
One issue with multi-view training with $n>1$ view is that the magnitude of noise after softmax decreases quadratically with respect to the number of views.
To illustrate this, similarly, consider $V' = V + N$ the value matrix to self-attention layer, with $V$ as the underlying information and $N$ as the noise.
Self-attention could be expressed as $W^\top V' = W^\top V + W^\top N$.
Assuming the noise $N$ has a zero mean, hence $var(W^\top N)= W^\top var(N)W$. In the case of $n$ views, in the extreme case where $W$ has uniform weights, the variance is $1/n^2$ smaller. Meanwhile, as $W$ is normalized, we can easily show $var(W^\top N) < var(N)$. 
}

\end{comment}


==> sections/4-system-eccv.tex <==
\section{Remaining system details}
\label{sec:details}
This section explains the remaining system details on the data preparations, the mesh extraction process, the MVAE pre-fine-tuning, and the three-stage training strategy.

\subsection{Training data preparation}
%\mypara{Multi-view cases}
Out of 800k 3D object models from Objaverse~\cite{deitke2023objaverse}, we use 180k models whose aesthetic scores~\cite{ava} are at least 5 for training.
%We prepare our training data using Objaverse~\cite{deitke2023objaverse} by filtering 180k objects from the full 800k dataset. Concretely, we compute the aesthetic score~\cite{ava} for each object using one rendered image and only keep objects with a score larger than 5 for training.
%
%All the images and their masks are encoded into 64×64 latents with the M-VAE.
%during training and generation. The training images are rendered from Objaverse~\cite{deitke2023objaverse}, and the foreground masks are readily available. 
For each object 3D model, we translate the bounding box center to the origin and apply uniform scaling so that the longest dimension matches $[-1, 1]$. The output camera centers are placed at a distance of 1.5 from the origin.
%(See \S\ref{subsec:camera} for the remaining details of the output camera configuration).
%The configuration of the rendering views are 
%The rendering of the training data follows the camera configuration 
%described in \S\ref{subsec:camera}. 
Input condition views are chosen in a similar way as Zero-123~\cite{liu2023zero}. 
Concretely, an azimuth angle is randomly chosen from one of the eight discrete angles of the output cameras (also see \S\ref{subsec:camera}). The elevation angle is set randomly from [-10$^\circ$, 45$^\circ$]. The distance of the camera center from the origin is set randomly from [1.5, 2.2]. We use Blender to render images. 

%For the reference view, we use the same azimuths while the elevation is randomly sampled from [-10$^\circ$, 45$^\circ$]. 

%Specifically, The elevation of the conditional view is randomly sampled from [-10$^\circ$, 45$^\circ$], and the radius (distance away from the center) is randomly sampled from [1.5, 2.2]. All the rendered images are with resolution 512$\times$512. We prepare the testing data using the GSO dataset, and the rendering details are provided in Sec.~\ref{exp_sec}.





\subsection{Testing data preparation}
\mypara{Single-view cases}
Google Scanned Object (GSO)~\cite{downs2022gso} is our testing dataset, where we borrow the rendered images and the evaluation pipeline
%We directly borrow the test data and evaluation pipelines from 
from SyncDreamer~\cite{liu2023syncdreamer}. Concretely, the test set consists of 30 objects. Each object has 16 images with a fixed elevation of 30$^\circ$ and every 22.5$^\circ$ for azimuth. SyncDreamer selected condition images by ``visual plausibility", which we copy. The details are provided in the supplementary. 
Since the azimuth angles in our training setting are every 45$^\circ$, eight images (starting from and including the condition image) are used for evaluation. The resolution of the rendered images is 256x256, while the image resolution of our architecture is 512x512. We upscale the condition images to 512x512 for our system inputs. The ground-truth images are 256x256 and we downscale our generated images to 256x256 for evaluation, while 512x512 images are used for the mesh reconstruction.
The Chamfer Distances (CD) and volume IoU between the ground-truth and reconstructed shapes are reported for single-view 3D reconstruction. The PSNR, SSIM~\cite{wang2004ssim}, and LPIPS~\cite{zhang2018lpips} are reported for novel view synthesis (NVS) 
%Note that only the first 8 views in our camera configuration overlap with SyncDreamer's 16 views (i.e., with azimuths 0$^\circ$, 45$^\circ$, $\dots$, 315$^\circ$, and elevation 30$^\circ$),
%we compute the NVS results of our method 
by averaging over the eight images.

\mypara{Sparse-view cases}
Sparse-view un-posed condition is a new setup (except the work of LEAP~\cite{jiang2023leap} and PF-LRM~\cite{wang2023pf-lrm} to our knowledge). We use a process similar to the single-view setting to render images.
%
Concretely, we first 
%Similar to the process of rendering the training data from Objaverse, 
render 10 condition images for each of the 30 GSO objects. The azimuth and the elevation angles are chosen randomly from [0, 360) and [-10, 45] respectively. 
% used in \S\ref{subsec:exp-single}.
%One difference is that the reference image's elevation is sampled from [-10$^\circ$, 45$^\circ$] . 
We render 32 ground-truth target images while aligning the azimuth of the first target view and the first input view (See \S\ref{subsec:camera}). The same evaluation metrics are used, while we vary the number of condition images to be 1, 2, 4 and 10.


% The azimuths are 0$^\circ$, 45$^\circ$, 90$^\circ$, $\dots$, 315$^\circ$, where the 0$^\circ$ is determined by the reference view. This camera configuration yields 32 generated images densely covering the object.


\subsection{Mesh extraction from generated images}
After generating 32 images, a neural implicit reconstruction method recovers a mesh model, similar to SyncDreamer~\cite{liu2023syncdreamer} and Wonder3D~\cite{long2023wonder3d}.
Specifically, we use grid-based NeuS~\cite{instant-nsr-pl,li2023neuralangelo}, where the foreground masks are decoded from the latent images $\{Z_i(0)\}$ by MVAE.
%Concretely, we train a grid-based NeuS~\cite{instant-nsr-pl,li2023neuralangelo} for each object using all the generated images and foreground masks.
%The masks are directly decoded from the latents by our M-VAE.
Since our generated images have high resolution and quality, we directly run the monocular normal estimator released by Omnidata~\cite{eftekhar2021omnidata} to obtain additional normal supervisions for NeuS without a normal generation module like Wonder3D. We borrow the NeuS implementation from Wonder3D's official codebase but do not use their ranking-based loss.
With a single Nvidia 2080 Ti, it takes around 3 minutes to reconstruct a textured mesh model.
The mesh could directly use the exported vertex color or be re-textured with the generated images. 



\subsection{Mask-aware VAE pre-fine-tuning}
We copy the network architecture and model weights of the default VAE~\cite{rombach2022high} and add additional input and output channels to handle the mask.
We found that fine-tuning Mask-aware VAE (M-VAE) only with object images improves performance.
%
%, which initializes the UNet input.
%at the first UNet block.
%We fine-tune M-VAE as a pre-processing
%e fine-tune the VAE 
%for the following two purposes: 1) Simultaneously modeling of foreground mask, and 2) improving reconstruction quality on object-centric images. 
%
Concretely, we use approximately 3 million RGBA images rendered from Objaverse to fine-tune M-VAE as a pre-processing. We follow the original VAE hyperparameters with a base learning rate of 4.5e-6 and a batch size of 64. The training runs for 60,000 iterations.
%
%This fine-tuning uses images from Objaverse, leveraging the LDM codebase
The binary cross entropy loss is used for the mask channel. The process improves PSNR from 36.6 to 41.2.
%For more details, see the \supp section. The enhanced VAE is referred to as M-VAE.


==> sections/5-exp-eccv.tex <==
\section{Experiments}\label{exp_sec}
% This section presents the experimental results of MVDiffusion++. 
%focuses on sparse view reconstruction outcomes.

%\subsection{Implementation details}\label{imple}
%\yasu{ training details is one massive paragraph. Is it possible to have some structure here (maybe combined with testing details contents?)}


We train the model with a batch size of 1024 using 128 Nvidia H100 GPUs for about a week. 
At test time, we use DDPM~\cite{ho2020denoising} sampler with 75 steps to sample the multi-view images, and it takes our model 30s, 77s, 123s, and 181s to generate 8, 16, 24, and 32 images, respectively.  
%
The section presents 
%the implementation details in Section~\ref{imple}, 
the single view experiments in \S\ref{subsec:exp-single}, the sparse view experiments in \S\ref{subsec:exp-sparse}, and text-to-3D application experiments
% the real-world examples
in \S\ref{subsec:text_to_3d}.

%\mypara{Others} As suggested by Zero123++~\cite{shi2023zero123++}, we use the linear noise schedule to replace the original scaled linear schedule of latent diffusion models and employ the v-prediction model~\cite{salimans2022progressive}. 



%\mypara{Evaluation} \yasu{this paragraph does not seem to add information} Following the evaluation pipeline of previous works~\cite{liu2023zero,liu2023syncdreamer,long2023wonder3d}, we evaluate our method on the Google Scanned Objects (GSO) dataset~\cite{downs2022gso} and compare it with various existing works. In the literature, single-view and sparse-view object modeling methods are mostly separate, so we divide our evaluation into two parts: \S\ref{subsec:exp-single} is for single-view object modeling, where we borrow the test settings from SyncDreamer~\cite{liu2023syncdreamer}; \S\ref{subsec:exp-sparse} is for sparse-view object modeling, where we construct a more challenging test setting and render the test images by ourselves.





\input{sections/5.1-single-view-exp-eccv}

\input{sections/5.2-sparse-view-exp}

\input{sections/5.3-text-to-3d}






==> sections/5.1-single-view-exp-eccv.tex <==
\subsection{Single-view object modeling}
\label{subsec:exp-single}
\input{tables/single_view_syncdreamer_setting}
%\mypara{Evaluation settings}
\input{figures/single_images_qualitative}
%
%\mypara{Baselines}
Three state-of-the-art single-view object modeling methods are our main baselines: SyncDreamer~\cite{liu2023syncdreamer}, Wonder3D~\cite{long2023wonder3d}, and Open-LRM~\cite{openlrm}. Since the evaluation pipeline is the same as SyncDreamer, we copy numbers of other baselines in their paper for comparison, which includes Zero123~\cite{liu2023zero}, RealFusion~\cite{melas2023realfusion}, Magic123~\cite{qian2023magic123}, One-2-3-45~\cite{liu2023one}, Point-E~\cite{nichol2022point}, and Shap-E~\cite{jun2023shap}. The following introduces the three main baselines and how we reproduce their systems:
%obtain their results:

\noindent \raisebox{0.25ex}{\tiny$\bullet$} {\it SyncDreamer} generates 16 images from fixed viewpoints given a single input image. The image resolution is 256x256. Their denoising network $\model$ initializes from Zero123 and leverages 3D feature volumes and depth-wise attention to learn multi-view consistency. 
It requires users to provide the elevation of the input image. 

\noindent \raisebox{0.25ex}{\tiny$\bullet$} {\it Wonder3D} takes a single input image as the canonical view and generates 6 images as well as the normal maps. The image resolution is 256$\times$256. Multi-view self-attention and an extra cross-domain attention ensure the consistency of generation results, while the views are sparser than ours.  We run the official codebase on the GSO input images to get the results. However, the released model assumes orthographic cameras and we cannot use the same test set to evaluate the NVS performance. ICP aligns the reconstructed mesh with the ground truth before computing the metrics.  

\noindent \raisebox{0.25ex}{\tiny$\bullet$} {\it Open-LRM} is an open-source implementation of Large Reconstruction Model (LRM)~\cite{hong2023lrm}, a generalized reconstruction model that predicts a triplane NeRF from a single input image using a feed-forward transformer-based network. ICP aligns the reconstructed mesh with the ground truth before computing the CD and volume IoU.

\input{figures/single_mesh_qualitative}


\mypara{Results} \autoref{tab:single-view-sync} presents the quantitative evaluations of the reconstructed 3D meshes and the generated images. \ourmethod~consistently outperforms all the competing methods with clear margins. Note that the evaluation is not completely fair for Wonder3D that assumes orthographic camera projections, where perspective images are used in the experiments. However, we believe the clear performance gaps suffice to demonstrate the strength of our method.     


\autoref{fig:single-images-qualitative} and \autoref{fig:single-mesh-qualitative} show generated images and reconstructed mesh models. In \autoref{fig:single-images-qualitative}, our method clearly shows the number on the clock (row 3), while others exhibit blurry numbers. In \autoref{fig:single-mesh-qualitative}, our method can recover a plausible and detailed shape of the turtle example (row 1), while Wonder3D and OpenLRM fail to recognize it as a turtle and exhibit significant artifacts. 
% In addition, for the board example (row 3), the design of MVAE of our method achieves precise mask segmentation, which leads to a clear and accurate 3D model, while the inaccurate segmentation of Wonder3D and Syncdreamer struggle results in inaccurate shapes and missing details.
%
%\ourmethod~demonstrate intricate details such as texts or complex textures 
%allows higher resolution, intricate details such as texts or complex textures can be better preserved in both generated images and reconstructed meshes
%\yasu{Look at figures and add 2 or 3 interesting things. Focus on writing things for specific examples instead of trying to write some high-level common comments for all the examples, which is difficult.}
%are the qualitative comparisons for the generated images and reconstructed meshes. Since \ourmethod~allows higher resolution, intricate details such as texts or complex textures can be better preserved in both generated images and reconstructed meshes. Furthermore, SyncDreamer and Wonder3D rely on an external segmentation tool to obtain the foreground mask for each generated image, but their default segmentation library could fail for some images and lead to noisy reconstruction results. In contrast, our method directly decodes the mask from the latents together with the image, producing cleaner mesh and simplifying the overall pipeline.    


==> sections/legacy/0-abs-old-0210.tex <==
\begin{abstract}
This paper presents a neural architecture {\ourmethod}~for 
%sparse-view
3D object reconstruction that synthesizes dense and high-resolution views of an object given one or a few images without camera poses as a condition. 
\ourmethod~achieves superior \textit{flexibility} and \textit{scalability} with two simple ideas
: 1) A ``pose-free architecture'' where standard self-attention among 2D latent features learns 3D consistency across arbitrary number of conditional and generation views without explicitly using camera pose information; and 2) A ``drop-view training strategy'' that simply discards a substantial number of output views during training, 
%view-level uniform dropout that drops a consistent set of views across layers, 
reducing the memory footprint for training and enabling dense and high-resolution view synthesis at test time.
%enabling us to reduce the training-time memory footprint and achieve dense and high-resolution view synthesis.
We use the Objaverse for training and the Google Scanned Objects for evaluation with standard novel view synthesis and 3D reconstruction metrics, where \ourmethod~significantly boosts over the current state of the arts. We also provide extensive qualitative results with in-the-wild images. The project page is \url{https://mvdiffusion-plusplus.github.io}.


%Extensive evaluations demonstrate that \ourmethod~excels in novel view synthesis and generalizes to in-the-wild objects, and enables high-quality single or sparse-view object reconstructions. 
\end{abstract}


% \begin{abstract}
% This paper introduces UniRecon, a unified framework to reconstruct objects from an arbitrary number of images in a pose-free manner. UniRecon generates dense multi-view images of fixed viewpoints with a conditional multi-view diffusion model, and those images can then be used to reconstruct object meshes. At the heart of UniRecon is a multi-branch stable-diffusion-impainting model, which reuses the pretrained stable diffusion self-attention to establish multi-view consistency between 1) generated images and 2) generated images and conditional images. UniRecon achieves state-of-the-art performance in both single-view and sparse-view object reconstructions. In the dense-view setting, xx 
% \end{abstract}

==> sections/legacy/1-intro-old-0210.tex <==
\section{Introduction}

\input{figures/teaser}


% \cjc{Since the millennium, the rapid evolution of the digital camera industry has enabled the capture of high-quality images at any time and place, producing exponentially increasing pixels. With 3D reconstruction algorithms that handle camera models and epipolar geometry, people have successfully extracted 3D models of objects~\cite{}, buildings~\cite{}, or even cityscapes~\cite{} from collections of photographs. Recently, the emergence of powerful text-to-image diffusion models~\cite{rombach2022StableDiffusion,saharia2022photorealistic,ramesh2022hierarchical} created chances for a family of more general reconstruction-by-generation algorithms. Specifically, these algorithms first generate multiple consistent images with a multi-view diffusion model~\cite{liu2023syncdreamer,shi2023zero123++,long2023wonder3d,liu2023one,liu2023one2345++}, and then convert them to 3D by predicting or training neural implicit fields~\cite{mildenhall2020nerf,wang2021neus}.

% However, these reconstruction-by-generation methods still suffer from limitations in two aspects. \textit{Flexibility:} They usually take a single image, while practical use cases might present an arbitrary number of photographs. \textit{Scalability:} The generated images are either sparse or low-resolution, thus having trouble covering the entire object or retaining the fine details of the input images. This paper proposes \ourmethod, which resolves 
% }

Diffusion-based generative models~\cite{ho2020denoising,song2020score-dm,song2019ncsn} have revolutionized high-resolution 2D image generation with seminal works such as Imagen~\cite{saharia2022photorealistic}, DALL-E~\cite{ramesh2022hierarchical}, and latent Diffusion~\cite{rombach2022high}. Building on this success, exciting developments in multi-view image generation emerged recently~\cite{tang2023mvdiffusion,shi2023mvdream,liu2023syncdreamer,long2023wonder3d,shi2023zero123++,liu2023one2345++}, with a focus on generating multiple images that are consistent across various viewpoints. 
% This consistency is crucial for object generation and scene creation applications, where different angles and perspectives are essential for a holistic representation. 
By ensuring multi-view consistency, the generated images can be seamlessly integrated into many downstream tasks, enhancing the realism and effectiveness of virtual environments, 3D modeling, and other advanced applications in gaming, virtual reality, and augmented reality.

MVDiffusion~\cite{tang2023mvdiffusion}, an early attempt to extend pre-trained text-to-image diffusion models to multiple images, generates high-resolution multi-view images to form a panorama or texturize a mesh by inserting lightweight correspondence-aware attention modules to a pre-trained diffusion UNet~\cite{rombach2022StableDiffusion}.
However, MVDiffusion requires pixel correspondences across views and does not handle arbitrary camera poses where 3D reasoning is essential.
%but is limited to scenarios where pixel-to-pixel correspondences are given across views.
%cannot extend to general cases due to the inability of handling occlusions. 
In succeeding works, more generalized cross-view attention is employed by MVDream~\cite{shi2023mvdream} and Wonder3D~\cite{long2023wonder3d}, which extends the original self-attention modules of diffusion UNet to operate on all image patches across views. 



This enhancement leads to
% enables these models to generate
multiple consistent images of an object, conditioned on a textual description or a single image. However, 3D self-attention demands high computational resources despite its power for view consistency.
% , while beneficial for view consistency, .
Consequently, these models are restricted to generating sparse and low-resolution images.
% producing images that are sparse and low-resolution. 
Furthermore, their applications are limited to cases of a single conditional image, where more complex scenarios require conditioning with multiple images without camera poses that cannot be estimated reliably due to minimal visual overlaps.
%scenarios involving a single image; they lack the capability to condition on multiple sparse unposed images, where accurate poses are hard to obtain. 
%This restriction narrows their usability in more complex or dynamic scenarios where multiple image inputs are essential for generating comprehensive multi-view representations.


%creates the model of an object or a scene in 3D space from a set of 2D measurements. These 2D measurements can be a set of point trajectories/matches~\cite{izadi2011kinectfusion, schonberger2016structure, agarwal2011building}, a single image~\cite{xu2019disn} or multiple images~\cite{yao2018mvsnet, furukawa2010towards}. They are utilized to define projections errors of scene structures and camera poses. However, these 2D measurements are sensitive to both photometric variance, such as lighting changes, and geometric variance, such as view point changes. More recent works learn to reconstruct 3D models of objects from image(s) end-to-end. Although they can tolerate larger view point changes, these learning-based methods usually have limited generalization capabilities, they either only handle a single object category~\cite{} or have sub-optimal performance across different categories and tend to degrade to retrieval~\cite{}[vladlen's paper]. 

This paper presents \ourmethod, a novel approach for generating
%a novel method \ourmethod, designed to generate 
dense and high-resolution multi-view images of an object, conditioned with a single or sparse input views without camera poses.
%. This method can handle inputs ranging from a single to multiple unposed images. 
%
Two simple ideas are at the heart of \ourmethod.
% Our approach centers around two key innovations.
First, we leverage a latent diffusion inpainting model~\cite{rombach2022StableDiffusion} with conditional and generation branches without explicitly using camera pose information or image projection formula.
%that are ``pose-free'' without explicitly using camera pose information or image projection formula.
Concretely, input conditional views are sparse without camera poses and are arbitrary, per example. Output generation views are fixed with known camera poses, but a learnable embedding per output view learns 3D consistency implicitly via a global attention mechanism without using camera poses or projection formula.
%First, we leverage a latent diffusion impainting model, which comprises two branches: a conditional branch and a generation branch. The conditional branch processes the input images, reconstructing them through a diffusion process. The other generation branch is responsible for creating dense images for fixed viewpoints. To link these images and ensure consistency, we utilize a global attention mechanism. 
%This system allows us to bypass the need for pose computation entirely, as all necessary correspondences are implicitly encoded within the network.
%
Second, we introduce ``view dropout'' training strategy, which randomly excludes generation views/branches in each batch, enabling the use of high-resolution images during training. During testing, this simple approach can surprisingly use all the branches and generate high-quality dense views.
%trick reduces memory consumption and enables the use of high-resolution images during training, while is capable of generating all the generation views at test time.

%1) it allows the model to be trained with a limited number of images, yet still capable of generating a variable number of high-resolution images during inference in a holistic manner. 2) by dropping redundant information, the model is encouraged to learn the global structure of the objects, resulting in higher image quality and multi-view consistency.



%Then, we can use conventional reconstruction algorithms to reconstruct objects from those generated images.

%3D reconstruction from a single or multiple images. Instead of relying on projection errors defined on points or images, we leverage the attention mechanism to find the correlation between images. We also represent a 3D object as multi-view RGB images from multiple canonical views, which enables us to leverage the diffusion model and guarantee the model can understand the underlying continuous distribution. These two designs enable us to learn a single network that unifies 3D reconstruction of objects from an arbitrary number of images and from any view-point. Specifically, we formulate the 3D reconstruction problem as a multi-view image generation problem. We leverage a latent diffusion impainting model, which are divided into a conditional branch and a generation branch. The conditional branch takes the conditional images and reconstruct the same image with diffusion process while the generation branch generates dense images at fixed viewpoints. We use a global attention mechanism to build correspondences among all the images. Then, we can use conventional reconstruction algorithms to reconstruct objects from those generated images.

\ourmethod achieves state-of-the-art performance on the task of novel view synthesis, single view reconstruction, and sparse view reconstruction. For single view reconsturction, our method achieves 0.6973 IoU and 0.0165 Chamfer distance on Google scanned object dataset, higher than syncdreamer~\cite{liu2023syncdreamer} by 0.1552 in terms of Vol. IOU. For novel view synthesis in sparse view setting, \ourmethod improve the PSNR by 8.19 compared with the recent paper LEAP~\cite{jiang2023leap}.
%Compared with previous methods, this approach does not require pose computation. All the correspondences are encoded into the network implicitly. Therefore, our Uni3D marriage the correspondence based multi-view geometry method and end-to-end learning based method, leading better robustness to photometric and geometric variance without trading the accuracy off. Our methods achieve state-of-the-art performance on both single and  sparse-view reconstruction. In addition, our simple and effective framework offers easy extendability, and can serve as a baseline for future researches.
% Previous works~\cite{} 
% .To this end, we propose the 

% Reconstructing a 3D object from a single image is crucial for applications like augmented and virtual reality (AR/VR), game design, and robotic simulations. This task, known as single-image 3D reconstruction, enables the creation of immersive experiences, the rapid prototyping of digital assets, and the enhancement of real-world interactions through simulations. However, it poses significant challenges due to the inherent ambiguity of inferring three-dimensional data from a two-dimensional source.

% Recent advancements in generative models have marked a significant milestone in this task. Zero-1-to-3~\cite{} generates perspective images of different viewpoints from conditional images with the diffusion model, and the 3D object can be distilled using score distillation loss~\cite{}. Based on zero-1-to-3, Syncdreamer proposes to generate multi-view images of fixed camera poses, and the generated images can be used to reconstruct objects using conventional reconstruction algorithms like Neus~\cite{}. These methods suffer from inconsistency issues because the concatenation of conditional images and noisy latent causes pixel misalignment between conditional images and generated images. In addition, the generated images are not dense enough to cover every viewpoint of the 3D objects.

% To address the above issue, PolyhedricFusion generates 36 images across two elevations (30, -30), 18 views for each elevation. Our core technique is to re-use the pretrained stable diffusion attention mechanism to align pixels of all the images, including both generated images and conditional images. Unlike the global 3D self-attention proposed in MVDream, we propose an efficient attention mechanism that divides the global 3D self-attention into cross-elevation attention and cross-azimuth attention and fuse them together into one block. 






==> sections/legacy/3-preliminary_old.tex <==
\section{Preliminary}
\label{sec:preliminary}
\ourmethod~ comprises multiple branches of an image latent diffusion model. The section will review latent diffusion models and their multi-view formulation, including our prior approach MVDiffusion~\cite{tang2023mvdiffusion}.

%architecture is built with multiple branches of image generative model
%latent diffusion image generative model
%including our prior system MVDiffusion~\cite{tang2023mvdiffusion}
%a multi-view diffusion model built upon the single-view latent diffusion models. We briefly review latent diffusion models and its multi-view formulation in this section.

\mypara{Latent diffusion models}
Latent Diffusion Model (LDM)~\cite{rombach2022StableDiffusion} has been a core machinery in the recent explosion of content generation techniques. 
LDM consists of a variational autoencoder (VAE)~\cite{kingma2013vae} with encoder $\encoder$ and decoder $\decoder$, a denoising network $\model$, and a condition encoder $\conditioner$. 
Raw images $\img \in \mathbb{R}^{\hpixel \times \wpixel \times \cpixel}$ are mapped to a compressed latent space by $\latent=\encoder(\img)$, $\latent \in \mathbb{R}^{\hlatent \times \wlatent \times \clatent}$, and the latents are converted back to image by $\imgrec = \decoder(\latent)$. 
The training objective is defined as
\begin{align}
\lsimpleldm := \expec_{ \encoder(\img), \cond, \bepsilon \sim \mathcal{N}(0, 1), t }\Big[ \Vert \bepsilon - \model(\latent_{t},t, \conditioner(\cond)) \Vert_{2}^{2}\Big] 
\label{eq:cond_ldm_loss}
\end{align}
where $t$ is uniformly sampled from $1$ to $T$ and $\latent_{t}$ is the noisy latent at time step $t$. The denoising network $\model$ is a UNet~\cite{dhariwal2021guided-diffusion} augmented with cross-attention mechanisms to incorporate the time embedding and the optional condition encoding $\conditioner(\cond)$. 
At sampling time, the reverse process generates samples in the latent space with advanced samplers~\cite{song2020ddim,karras2022edm}, and the VAE decoder outputs final images with a single forward pass. 


\mypara{Multi-view latent diffusion models} Recent 3D modeling works have fine-tuned LDM to generate consistent multi-view images, conditioned either on a text description or an image~\cite{tang2023mvdiffusion,shi2023mvdream,liu2023syncdreamer,shi2023zero123++}. Two fundamental extensions are made to adapt a pre-trained LDM to multiple images: 1) the forward process injects noises into all the image latents, and 2) the denoising network is modified to take all the noisy latents and denoise them simultaneously. The general training objective of the multi-view LDM can be defined as
\begin{align}
\lsimplemv
:= \expec_{\left\{\encoder(\img^i) \right\}_{i=1}^N, \left\{\bepsilon^i \sim \mathcal{N}(0, I)\right\}_{i=1}^N, \cond, t} \Big[ \sum_{i=1}^N \Vert \bepsilon^i - \model^i(\left\{ \latent_t^i \right\},t, \conditioner(\cond)) \Vert_{2}^{2}\Big].
\label{eq:cond_mvldm_loss}
\end{align}
Previous works mainly differ in the designs of the multi-view denoising network $\model$, including how the conditions are incorporated and how the information between multiple generated views is synchronized. The essential contributions of \ourmethod~are two-folded: 1) an inpainting-style formulation for $\model$, which flexibly takes any number of pose-free condition images and generates multi-view images, and 2) a simple yet effective training strategy, view dropout, which enables the model to generate dense multi-view images at higher resolutions. 





==> sections/legacy/4-method-old.tex <==
\section{\ourmethod}
\ourmethod~generates dense (32) and high-resolution (512$\times$512) images from single or multiple un-posed images. These high-fidelity generated images provide rich details of an object from almost all perspectives,
making them easily used for 3D reconstruction. 
% with NeRF~\cite{mildenhall2020nerf}, NeuS~\cite{wang2021neus}, or their variants. 
% The core of \ourmethod~is an inpainting-style multi-branch and multi-view diffusion model, initialized from latent Diffusion inpainting model~\cite{rombach2022high}. 
% Figure~\ref{fig:overview} shows an overview of the method, and 
This section is organized as follows: \S~\ref{subsec:camera} describes the camera configurations of the conditional and generated images. \S~\ref{subsec:vae-ft} introduces the VAE fine-tuning for simultaneous foreground mask modeling and less encoding information loss. \S~\ref{subsec:dm} and \S~\ref{subsec:view-drop} demonstrate our key innovations, the pose-free multi-view conditional diffusion model and the view dropout training strategy, respectively. Finally, \S~\ref{subsec:detail} discusses the training details and how we export meshes from the generated images.


\input{figures/generation_example}
\input{figures/method}

\subsection{Camera configuration}
\label{subsec:camera}
Figure~\ref{fig:generated_views} illustrates the camera settings of generated views in \ourmethod, based on which we also render Objaverse~\cite{deitke2023objaverse} objects to prepare our training data.
%
For each object, we first render 10 input images from random viewpoints and pick one as the reference view. We then prepare the generation targets based on the reference view, following a fixed pattern of elevations and azimuths. Specifically, there are four different elevation levels and eight different azimuth levels. The elevations are 60$^\circ$, 30$^\circ$, 0$^\circ$, and -30$^\circ$ in the default object coordinate system of Objaverse where all objects are upright and z-axis aligned. The azimuths are 0$^\circ$, 45$^\circ$, 90$^\circ$, $\dots$, 315$^\circ$, where the 0$^\circ$ is determined by the reference view. This camera configuration yields 32 generated images densely covering the object. During training, the conditional images are randomly sampled from the 10 input images while the reference view is always picked.



% Given a collection of $N$ images rendered from random viewpoints, one image is chosen as the reference. The generation of new images is based on this reference, following a fixed pattern of elevations and azimuths. Specifically, the elevations are set at 60, 30, 0, and -30 degrees. For azimuth, the increments are every 45 degrees. This systematic approach results in 32 distinct images densely covering an object. The azimuth values are determined relative to the chosen reference image, while the elevation values are pre-established in the training dataset, Objaverse, where all the objects are upright and z-axis aligned.

\subsection{Mask-aware VAE fine-tuning}
\label{subsec:vae-ft}

Before training the multi-view diffusion model, we propose to first fine-tune the VAE for the following two purposes:
\begin{enumerate}
[label={ {(\arabic*).}},leftmargin=*,topsep=0.5ex,itemsep=-0.5ex,partopsep=0.75ex,parsep=0.75ex,partopsep=0pt,wide, labelwidth=!,labelindent=0pt]
\item {\bf Simultaneously modeling of foreground mask.} When exporting the mesh from generated multi-view images, recent methods (e.g., SyncDreamer~\cite{liu2023syncdreamer} and Wonder3D~\cite{long2023wonder3d}) rely on an external segmentation model to produce accurate foreground masks, and the mask quality is vital for reconstruction quality. However, the mask information could have been captured by the rich LDM latents~\cite{wu2023datasetdm}, and simultaneous modeling of the image and the foreground mask is possible. We remove this external dependency by adding an extra input and output channel to the original VAE from the pre-trained LDM. 
\item {\bf Reducing compression rate for multi-view consistency.} VAE encoding is a lossy process and leads to inconsistencies among the multi-view latents, and the issue becomes more serious when the number of conditional and generated images increases. Therefore, we fine-tune the VAE to increase the PSNR of the reconstructed images.
\end{enumerate}

% \input{tables/vae_results}

% In summary, we fine-tune the VAE to enable simultaneous modeling of foreground mask and reduce the compression rate, and 


The fine-tuning is conducted with images from Objaverse. We use the original codebase of LDM~\cite{rombach2022StableDiffusion}, and binary cross entropy is the reconstruction loss for the mask channel. We convert the fine-tuned VAE checkpoint to Diffusers using its official conversion script. Please check the \supp~for complete details. We denote the fine-tuned mask-aware VAE with M-VAE.

% \footnote{\url{https://github.com/huggingface/diffusers/blob/main/scripts/convert_vae_pt_to_diffusers.py}}


% The traditional methods of reconstruction rely on accurate foreground masks, typically obtained using segmentation techniques like SAM. However, these methods struggle when the masks are imprecise. Moreover, the pre-trained stable diffusion models show a significant reconstruction error in the objaverse dataset, attributed to a domain shift. To address these issues, we modify the Variational Autoencoder (VAE) to process both RGB images and mask information. This refinement involves adding an extra input and output channel to the original stable diffusion VAE. This modification enables the encoding and decoding of the foreground/background mask alongside the RGB image. The encoder transforms the RGB-mask image into a four-channel latent space, which is downsampled by a factor of 8. The decoder then reconstructs this latent space back into the original RGB-mask format. For the RGB channels, we maintain the use of mean square error, GAN loss, and LPIP loss as training objectives. In contrast, for the mask channel, binary cross-entropy loss is employed for optimization. We present in Table~[reference needed] a comparative analysis of the Peak Signal-to-Noise Ratio (PSNR) and segmentation Intersection Over Union (IOU) between the fine-tuned model and the pre-trained model. For evaluating the segmentation mask on the pre-trained stable diffusion VAE, we utilize [method/technique needed] to segment the foreground/background mask on the reconstructed images. The results demonstrate a substantial improvement in performance with the fine-tuned VAE.


\subsection{Pose-free multi-view conditional diffusion model}
\label{subsec:dm}


We employ the general framework of multi-view LDM as described in \S\ref{sec:preliminary} and focus on proposing a more flexible architecture for the multi-view denoising network $\model$. Compared to previous multi-view diffusion models such as MVDiffusion~\cite{tang2023mvdiffusion}, SyncDreamer~\cite{liu2023syncdreamer}, or Wonder3D~\cite{long2023wonder3d}, etc, our architecture has two unique advantages: 
1) we allow the model to take an arbitrary number of input views (1-10), making the model suitable for both single and sparse-view conditioning; 2) the model does not require camera poses, refraining us from the challenging pose estimation process when input images are sparse and have limited overlaps.

Inspired by the image-to-panorama variant of MVDiffusion~\cite{tang2023mvdiffusion}, our denoising network $\model$ is formulated as an inpainting-style model and initialized from latent Diffusion's inpainting model. Figure~\ref{fig:overview} provides an illustration of the architecture. The model consists of two branches: a \textit{conditional branch} to digest single or sparse-view inputs, and a \textit{generation branch} to synthesize consistent dense multi-view images at fixed viewpoints with respect to the reference view.  
%
Each conditional or generated image is processed individually by a copy of the UNet, while the input of the UNet consists of three parts: 1) the noisy latents; 2) a binary mask to distinguish the conditional and generated images (all ones for conditional images and all zeros for generates images); and 3) the condition latents, which is the encodings of the conditional images for the conditional branch, and the encodings of pure-white images for the generation branch. The three parts are concatenated following the inputs of pretrained latent impainting model before passing to the UNet. 

We use learnable view embeddings to distinguish different images. The condition branch has two learnable view embeddings: $\tau(C_{r})$ is assigned to the reference view $C_{r}$, and $\tau(C_{d})$ is assigned to all other conditional views. Each fixed viewpoint 
in the generation branch has a unique learnable embedding $\tau(C_{i})$, $i=1,\dots,32$. As shown by Figure~\ref{fig:overview}, the view embeddings are added to the timestep embedding $\tau(t)$ and injected into each UNet copy. 
We multiply the view embeddings by a zero-initialized trainable scale $\alpha$ to avoid model disruption at initialization. 

% The view embedding is injected into the UNet following the same manner as the timestep embedding.
% \begin{equation}
 % T=T_{time}+\alpha T_{view}
% \end{equation}

Inspired by MVDream~\cite{shi2023mvdream}, all UNet copies from the two branches are interconnected by self-attention mechanisms among the patch-level latent tokens. The self-attention blocks from the original latent diffusion models~\cite{rombach2022StableDiffusion} are reused to learn multi-view 3D consistencies between all conditional and generated images. Concretely, for a batch of $B$ samples with each having $N$ conditional images and $M$ generation images, the tensor size for the two branches would be $[B,N,C,H,W]$ and $[B,M,C,H,W]$, respectively, where $C, H, W$ are the number of channels, height, and width of the UNet features at a specific self-attention layer. We concatenate and reshape these tensors into a new tensor of size $[B,(N+M)*H*W,C]$, then apply global self-attention at the second dimension. This global multi-view attention is expected to learn three-level relations to enforce multi-view consistency: 1) between conditional images; 2) from conditional images to generation images; 3) between generation images.


The huge computation cost used to be a core limitation for the above multi-view global attention, but thanks to the progress in memory-efficient transformers for large language models~\cite{dao2022flashattention,dao2023flashattention2}, state-of-the-art attention techniques can already afford a large number of tokens. Using the attention implementations in Diffusers~\cite{diffusers} together with our view dropout training strategy (described in \S\ref{subsec:view-drop}), our multi-view conditional diffusion model manages to take up to 10 conditional images and generate 32 dense images, all at resolution 512$\times$512, providing broader coverage and richer details for the objects. 





\begin{comment}
Our approach begins with encoding the conditional images into a latent space using a Variational Autoencoder (VAE) and apply diffusion model to generate multi-view images based the encoded latents. The design of our model is inspired by MVDifusion~\cite{tang2023mvdiffusion} and consists of two primary branches: the \textit{conditional branch} and the \textit{generation branch}. Both branches are underpinned by a stable diffusion inpainting model framework, which serves as the foundation for our architecture.

The conditional branch is tasked with processing the latents of the conditional images. Here, each latent image is individually fed through a separate stable diffusion Unit. This Unit is designed to handle a noisy latent input, initially comprising Gaussian noise. This noise is combined with the latent of a conditional image and a mask filled entirely with ones. The UNet then predicts velocity (v-prediction) in a diffusion process to reconstruct the latent of the conditional image. In practice, we set the number of conditional images to be ranged from 1 to 10. To handle variable input, we repeat the first reference image multiple times to form a constant 10 conditional images.

The generation branch is specifically focused on generating images from novel viewpoints. The detailed camera settings for this branch are outlined in Section~\ref{subsec:camera}. In this branch, the UNet initiates with a base of Gaussian-initialized noise. This noise is then concatenated with a zero-initialized latent and a zero mask. 

Following MVDream, we reuse the 2D self-attention mechanism from the stable diffusion (SD) Unet with a 3D self-attention mechanism. This integration is pivotal in establishing connections between the images in both the conditional and generation branches. For instance, assuming we have $N$ conditional images and $M$ generation images, the tensor size for the conditional branch images would be $B N C H W$, and for the generation branch, $B M C H W$. We concatenate and reshape these tensors into a new tensor of size $B C (N+M) H W$, applying 3D self-attention to this concatenated tensor. The 3D self-attention mechanism is instrumental in building matches between all pairs of images and encoding cost volume information into the attention process, enhancing the model's capability to generate coherent and contextually aligned images.

We use a learnable camera embedding to differentiate different view-points. For conditional branch, we have two learnable camera embeddings: one is assigned to the reference images, while all the remaining conditional images use the other embedding. For the generation branch, we assign each view-point with a learnable embedding. The learnable embedding is added to time embedding in each Unet unit. The embedding is also multiplied by a zero-initialized scale to prevent model disruption at initialization.
\end{comment}

\subsection{View dropout}
\label{subsec:view-drop}

Based on the camera configuration and the model architecture described in \S~\ref{subsec:camera}  and \S~\ref{subsec:dm}, \ourmethod~needs to process up to 42 UNet copies (i.e., 10 conditional ones and 32 generated ones) in a single forward pass with global multi-view self-attention. Empirically, we find that training the model with this amount of high-resolution images presents two challenges:

\begin{enumerate}
[label={ {(\arabic*).}},leftmargin=*,topsep=0.5ex,itemsep=-0.5ex,partopsep=0.75ex,parsep=0.75ex,partopsep=0pt,wide, labelwidth=!,labelindent=0pt]

\item {\bf Computational feasibility.} Considering images with resolution 512$\times$512, each image latent has size 64$\times$64. 32 generated images and 1-10 conditional images will lead to more than 130K tokens for the multi-view self-attention in the first and last UNet block. Handling even a million tokens has become possible with advanced memory-efficient attention, but since the training of multi-view diffusion models usually requires much more memory usage, the training process of 42 views is not feasible even in the most power GPU in the world. 

\item {\bf Information redundancy.} The dense training views can lead to excess redundant signals, making it hard for the diffusion process to reduce the signal-to-noise ratio (SNR), which is similar to the case of training diffusion models for large images~\cite{chen2023importance_noise} or videos~\cite{blattmann2023stablevideodm}. Our early experiments showed that too-dense training views could hurt the generation quality even when we shift the noise schedule towards higher noise values, as suggested by previous works.
\end{enumerate}

To tackle these two issues, we propose a simple yet surprisingly effective strategy, \textit{view dropout}, a view-level uniform dropout that completely discards a set of views across all layers during training. We found even a large drop rate can work well in practice. Specifically, we randomly drop 24 out of 32 views for each object at each training iteration, which significantly reduces the training cost. At test time, the model is able to generate an arbitrary subset of the 32 views. Furthermore, due to the information redundancy issue discussed above, training with our view dropout leads to better generation quality than training with a full 32 views. We provide a tentative theoretical analysis in the \supp.


% To make this more manageable and efficient, we implement a strategy of dropping a considerable number of generation views during training. Specifically, for each training object, we randomly select $N$ images from a set of 32 pre-rendered images. These selected images, along with the conditional images, are then used to train each Unet unit. Importantly, 3D self-attention is applied across all these sampled views. During the inference phase, our model demonstrates the capability to generate an arbitrary number of views given the corresponding camera embeddings, with 3D self-attention applied to all these generated views. This method of view dropout is akin to the commonly used attention dropout technique in network training, serving as an effective regularization method. Empirically, we have found that even a small number of views (setting $N=8$) can yield satisfactory performance.


\begin{comment}

\dilin{
Very very brief explanation of view drop: 
Assuming $n$ noisy views $\{v'_i\}_{i=1}^n$ with each view $v'_i = v_i + \epsilon_i$, where $v_i$ is the underlying real information and $\epsilon_i$ is the noise.
One issue with multi-view training with $n>1$ view is that the magnitude of noise after softmax decreases quadratically with respect to the number of views.
To illustrate this, similarly, consider $V' = V + N$ the value matrix to self-attention layer, with $V$ as the underlying information and $N$ as the noise.
Self-attention could be expressed as $W^\top V' = W^\top V + W^\top N$.
Assuming the noise $N$ has a zero mean, hence $var(W^\top N)= W^\top var(N)W$. In the case of $n$ views, in the extreme case where $W$ has uniform weights, the variance is $1/n^2$ smaller. Meanwhile, as $W$ is normalized, we can easily show $var(W^\top N) < var(N)$. 
}

\end{comment}


\subsection{More details}
\label{subsec:detail}


\mypara{Training details}
As suggested by Zero123++~\cite{shi2023zero123++}, we use the linear noise schedule to replace the original scaled linear schedule of latent diffusion models and employ the v-prediction model~\cite{salimans2022progressive}. We also incorporate the Zero-SNR fix~\cite{lin2024common}  commonly adopted in video generation models. Note that our model is initialized from a $\epsilon$-prediction latent inpainting diffusion model, so it is necessary to adapt it into a v-prediction model via fine-tuning.  
In addition, training a single-view conditioning model is much more challenging than training a sparse-view conditioning one due to the higher uncertainty, and the former model can be easily fine-tuned to take multiple condition images.    
With the above observations, we employ a three-stage training strategy: 1)  We first train a single-view conditioning model with $\epsilon$-prediction, finetuning from the initial latent diffusion impainting model; 2) Subsequently, we shift the model to v-prediction and still train with single-view conditioning; 3) Finally, we finetune the model to integrate single and sparse-view conditioning. 
%
In the final stage, we use view paddings to handle joint single and sparse-view training, and we randomly assign half the samples to single-view conditioning and the other half to sparse-view settings for each iteration. We uniformly sample 2 to 10 views from the condition images for sparse-view conditioning.

All the images and their masks are encoded into 64×64 latents with the M-VAE during training and generation. The training images are rendered from Objaverse~\cite{deitke2023objaverse}
 and the foreground masks are readily available.
At test time, for conditional images in RGBA format, the alpha channel is converted to the mask; otherwise, we use Clipdrop~\cite{clipdrop} to get the foreground mask. 
We train the model with a total batch size 1024 using 128 Nvidia H100 GPUs. We employ an AdamW optimizer with a learning rate of 7e-5 and use a cosine learning rate scheduler similar to Zero123++. 


\mypara{Mesh extraction from generated images}
After generating the dense multi-view images (all views in Fig.~\ref{fig:generated_views}), we employ neural implicit reconstruction methods to extract the 3D geometry, similar to SyncDreamer~\cite{liu2023syncdreamer} and Wonder3D~\cite{long2023wonder3d}. Concretely, we train a grid-based NeuS~\cite{instant-nsr-pl,li2023neuralangelo} for each object using all the generated images and foreground masks. The masks are directly decoded from the latents by our M-VAE.
Since our generated images have high resolution and quality, we directly run the monocular normal estimator released by Omnidata~\cite{eftekhar2021omnidata} to get the extra normal supervision for NeuS without the need for a normal generation module like Wonder3D. We borrow the NeuS implementation from Wonder3D's official codebase but do not use their ranking-based loss.
With a single Nvidia 2080 Ti, it takes around 3 minutes to finish the NeuS training and export a textured mesh. 

==> sections/legacy/4-method_old_ver2.tex <==
\section{\ourmethod}
\ourmethod~generates dense (32) and high-resolution (512$\times$512) images from single or multiple un-posed images. These high-fidelity generated images provide rich details of an object from almost all perspectives,
making them easily used for 3D reconstruction. 
% with NeRF~\cite{mildenhall2020nerf}, NeuS~\cite{wang2021neus}, or their variants. 
% The core of \ourmethod~is an inpainting-style multi-branch and multi-view diffusion model, initialized from latent Diffusion inpainting model~\cite{rombach2022high}. 
% Figure~\ref{fig:overview} shows an overview of the method, and 
This section is organized as follows: \S\ref{subsec:camera} describes the camera configurations of the conditional and generated images. \S\ref{subsec:vae-ft} introduces the VAE fine-tuning for simultaneous foreground mask modeling and less encoding information loss. \S\ref{subsec:dm} and \S\ref{subsec:view-drop} demonstrate our key innovations, the pose-free multi-view conditional diffusion model and the view dropout training strategy, respectively. Finally, \S\ref{subsec:detail} discusses the training details and how we export meshes from the generated images.


\input{figures/generation_example}
\input{figures/method}

\subsection{Camera configuration}
\label{subsec:camera}
Figure~\ref{fig:generated_views} illustrates the  camera settings of generated views in \ourmethod, based on which we also render Objaverse~\cite{deitke2023objaverse} objects to prepare our training data.
%
For each object, we first render 10 input images from random viewpoints and pick one as the reference view. We then prepare the generation targets based on the reference view, following a fixed pattern of elevations and azimuths. Specifically, there are four different elevation levels and eight different azimuth levels. The elevations are 60$^\circ$, 30$^\circ$, 0$^\circ$, and -30$^\circ$ in the default object coordinate system of Objaverse where all objects are upright and z-axis aligned. The azimuths are 0$^\circ$, 45$^\circ$, 90$^\circ$, $\dots$, 315$^\circ$, where the 0$^\circ$ is determined by the reference view. This camera configuration yields 32 generated images densely covering the object. During training, the conditional images are randomly sampled from the 10 input images, while the reference view is always picked. All images are 512$\times$512.



\subsection{Pose-free multi-view conditional diffusion model}
\label{subsec:dm}


We employ the general framework of multi-view LDM as described in \S\ref{sec:preliminary} and focus on proposing a more flexible architecture for the multi-view denoising network $\model$. Compared to previous multi-view diffusion models such as MVDiffusion~\cite{tang2023mvdiffusion}, SyncDreamer~\cite{liu2023syncdreamer}, or Wonder3D~\cite{long2023wonder3d}, etc, our architecture has two unique advantages: 
1) we allow the model to take an arbitrary number of input views (1-10), making the model suitable for both single and sparse-view conditioning; 2) the model does not require camera poses, refraining us from the challenging pose estimation process when input images are sparse and have limited overlaps.

Inspired by the image-to-panorama variant of MVDiffusion~\cite{tang2023mvdiffusion}, our denoising network $\model$ is formulated as an inpainting-style model and initialized from latent Diffusion's inpainting model. Figure~\ref{fig:overview} provides an illustration of the architecture. The model consists of two branches: a \textit{conditional branch} to digest single or sparse-view inputs, and a \textit{generation branch} to synthesize consistent dense multi-view images at fixed viewpoints with respect to the reference view.  
%
Each conditional or generated image is processed individually by a copy of the UNet, while the input of the UNet consists of three parts: 1) the noisy latents; 2) a binary mask to distinguish the conditional and generated images (all ones for conditional images and all zeros for generates images); and 3) the condition latents, which is the encodings of the conditional images for the conditional branch, and the encodings of pure-white images for the generation branch. The three parts are concatenated following the inputs of pretrained latent impainting model before passing to the UNet. 

We use learnable view embeddings to distinguish different images. The condition branch has two learnable view embeddings: $\tau(C_{r})$ is assigned to the reference view $C_{r}$, and $\tau(C_{d})$ is assigned to all other conditional views. Each fixed viewpoint 
in the generation branch has a unique learnable embedding $\tau(C_{i})$, $i=1,\dots,32$. As shown by Figure~\ref{fig:overview}, the view embeddings are added to the timestep embedding $\tau(t)$ and injected into each UNet copy. 
We multiply the view embeddings by a zero-initialized trainable scale $\alpha$ to avoid model disruption at initialization. 

Inspired by MVDream~\cite{shi2023mvdream}, all UNet copies from the two branches are interconnected by self-attention mechanisms among the patch-level latent tokens. The self-attention blocks from the original latent diffusion models~\cite{rombach2022StableDiffusion} are reused to learn multi-view 3D consistencies between all conditional and generated images. Concretely, for a batch of $B$ samples with each having $N$ conditional images and $M$ generation images, the tensor size for the two branches would be $[B,N,C,H,W]$ and $[B,M,C,H,W]$, respectively, where $C, H, W$ are the number of channels, height, and width of the UNet features at a specific self-attention layer. We concatenate and reshape these tensors into a new tensor of size $[B,(N+M)*H*W,C]$, then apply global self-attention at the second dimension. This global multi-view attention is expected to learn three-level relations to enforce multi-view consistency: 1) between conditional images, 2) from conditional images to generation images, and 3) between generation images.


The huge computation cost used to be a core limitation for the above multi-view global attention, but thanks to the progress in memory-efficient transformers for large language models~\cite{dao2022flashattention,dao2023flashattention2}, state-of-the-art attention techniques can already afford a large number of tokens. Using the attention implementations in Diffusers~\cite{diffusers} together with our view dropout training strategy (described in \S\ref{subsec:view-drop}), our multi-view conditional diffusion model manages to take up to 10 conditional images and generate 32 dense images, all at resolution 512$\times$512, providing broader coverage and richer details for the objects. 


\subsection{View dropout}
\label{subsec:view-drop}

Based on the camera configuration and the model architecture described in \S\ref{subsec:camera}  and \S\ref{subsec:dm}, \ourmethod~needs to process up to 42 UNet copies (i.e., 10 conditional ones and 32 generated ones) in a single forward pass with global multi-view self-attention. Empirically, we find that training the model with this amount of high-resolution images presents two challenges:

\begin{enumerate}
[label={ {(\arabic*).}},leftmargin=*,topsep=0.5ex,itemsep=-0.5ex,partopsep=0.75ex,parsep=0.75ex,partopsep=0pt,wide, labelwidth=!,labelindent=0pt]

\item {\bf Computational feasibility.} Considering images with resolution 512$\times$512, each image latent has size 64$\times$64. 32 generated images and 1-10 conditional images will lead to more than 130K tokens for the multi-view self-attention in the first and last UNet block. Handling even a million tokens has become possible with advanced memory-efficient attention, but since the training of multi-view diffusion models usually requires much more memory than inference, the training process of 42 high-resolution images is not feasible even with the most powerful GPU in the world. 

\item {\bf Information redundancy.} The dense training views can lead to excess redundant signals, making it hard for the diffusion process to decrease the signal-to-noise ratio (SNR), which is similar to the case of training diffusion models for large images~\cite{chen2023importance_noise} or videos~\cite{blattmann2023stablevideodm}. Our early experiments showed that too-dense training views could hurt the generation quality even when we shift the noise schedule towards higher noise values following the suggestions of previous works.
\end{enumerate}

To tackle these two issues, we propose a simple yet surprisingly effective strategy, \textit{view dropout}, a view-level uniform dropout that completely discards a set of views across all layers during training. We found even a large drop rate can work well in practice. Specifically, we randomly drop 24 out of 32 views for each object at each training iteration, which significantly reduces the training cost. At test time, the model is able to generate an arbitrary subset of the 32 views. Furthermore, due to the information redundancy issue discussed above, training with our view dropout leads to better generation quality than training with a full 32 views. We provide a tentative theoretical analysis in the \supp.


% To make this more manageable and efficient, we implement a strategy of dropping a considerable number of generation views during training. Specifically, for each training object, we randomly select $N$ images from a set of 32 pre-rendered images. These selected images, along with the conditional images, are then used to train each Unet unit. Importantly, 3D self-attention is applied across all these sampled views. During the inference phase, our model demonstrates the capability to generate an arbitrary number of views given the corresponding camera embeddings, with 3D self-attention applied to all these generated views. This method of view dropout is akin to the commonly used attention dropout technique in network training, serving as an effective regularization method. Empirically, we have found that even a small number of views (setting $N=8$) can yield satisfactory performance.


\begin{comment}

\dilin{
Very very brief explanation of view drop: 
Assuming $n$ noisy views $\{v'_i\}_{i=1}^n$ with each view $v'_i = v_i + \epsilon_i$, where $v_i$ is the underlying real information and $\epsilon_i$ is the noise.
One issue with multi-view training with $n>1$ view is that the magnitude of noise after softmax decreases quadratically with respect to the number of views.
To illustrate this, similarly, consider $V' = V + N$ the value matrix to self-attention layer, with $V$ as the underlying information and $N$ as the noise.
Self-attention could be expressed as $W^\top V' = W^\top V + W^\top N$.
Assuming the noise $N$ has a zero mean, hence $var(W^\top N)= W^\top var(N)W$. In the case of $n$ views, in the extreme case where $W$ has uniform weights, the variance is $1/n^2$ smaller. Meanwhile, as $W$ is normalized, we can easily show $var(W^\top N) < var(N)$. 
}

\end{comment}


\section{Implementation details}
\label{sec:details}


\subsection{Mask-aware VAE fine-tuning}
\label{subsec:vae-ft}

Before training the multi-view diffusion model, we fine-tune the VAE for the following two purposes:
\begin{enumerate}
[label={ {(\arabic*)}},leftmargin=*,topsep=0.5ex,itemsep=-0.5ex,partopsep=0.75ex,parsep=0.75ex,partopsep=0pt,wide, labelwidth=!,labelindent=0pt]
\item {\bf Simultaneously modeling of foreground mask.} When exporting the mesh from generated multi-view images, recent methods (e.g., SyncDreamer~\cite{liu2023syncdreamer} and Wonder3D~\cite{long2023wonder3d}) rely on an external segmentation model to produce accurate foreground masks, and the mask quality is vital for reconstruction quality. However, the mask information could have been captured by the rich LDM latents~\cite{wu2023datasetdm}, and simultaneous modeling of the image and the foreground mask is possible. We remove this external dependency by adding an extra input and output channel to the original VAE from the pre-trained LDM. 
\item {\bf Reducing compression rate for multi-view consistency.} VAE encoding is a lossy process and leads to inconsistencies among the multi-view latents, and the issue becomes more serious when the number of conditional and generated images increases. Therefore, we fine-tune the VAE to increase the PSNR of the reconstructed images.
\end{enumerate}

% \input{tables/vae_results}

% In summary, we fine-tune the VAE to enable simultaneous modeling of foreground mask and reduce the compression rate, and 

\noindent
The fine-tuning is conducted with images from Objaverse. We use the original codebase of LDM~\cite{rombach2022StableDiffusion}, and binary cross entropy is the reconstruction loss for the mask channel. We convert the fine-tuned VAE checkpoint to Diffusers using its official conversion script. Please check the \supp~for complete details. We denote the fine-tuned mask-aware VAE with M-VAE.


\subsection{Training details}
As suggested by Zero123++~\cite{shi2023zero123++}, we use the linear noise schedule to replace the original scaled linear schedule of latent diffusion models and employ the v-prediction model~\cite{salimans2022progressive}. We also incorporate the Zero-SNR fix~\cite{lin2024common}  commonly adopted in video generation models. Note that our model is initialized from a $\epsilon$-prediction latent inpainting diffusion model, so it is necessary to adapt it into a v-prediction model via fine-tuning.  
In addition, training a single-view conditioning model is much more challenging than training a sparse-view conditioning one due to the higher uncertainty, and the former model can be easily fine-tuned to take multiple condition images.    
With the above observations, we employ a three-stage training strategy: 1)  We first train a single-view conditioning model with $\epsilon$-prediction, finetuning from the initial latent diffusion impainting model; 2) Subsequently, we shift the model to v-prediction and still train with single-view conditioning; 3) Finally, we finetune the model to integrate single and sparse-view conditioning. 
%
In the final stage, we use view paddings to handle joint single and sparse-view training, and we randomly assign half the samples to single-view conditioning and the other half to sparse-view settings for each iteration. We uniformly sample 2 to 10 views from the condition images for sparse-view conditioning.

All the images and their masks are encoded into 64×64 latents with the M-VAE during training and generation. The training images are rendered from Objaverse~\cite{deitke2023objaverse}
 and the foreground masks are readily available.
At test time, for conditional images in RGBA format, the alpha channel is converted to the mask; otherwise, we use Clipdrop~\cite{clipdrop} to get the foreground mask. 
We train the model with a total batch size 1024 using 128 Nvidia H100 GPUs. We employ an AdamW optimizer with a learning rate of 7e-5 and use a cosine learning rate scheduler similar to Zero123++. 


\subsection{Mesh extraction from generated images}
After generating the dense multi-view images (all views in Fig.~\ref{fig:generated_views}), we employ neural implicit reconstruction methods to extract the 3D geometry, similar to SyncDreamer~\cite{liu2023syncdreamer} and Wonder3D~\cite{long2023wonder3d}. Concretely, we train a grid-based NeuS~\cite{instant-nsr-pl,li2023neuralangelo} for each object using all the generated images and foreground masks. The masks are directly decoded from the latents by our M-VAE.
Since our generated images have high resolution and quality, we directly run the monocular normal estimator released by Omnidata~\cite{eftekhar2021omnidata} to get the extra normal supervision for NeuS without the need for a normal generation module like Wonder3D. We borrow the NeuS implementation from Wonder3D's official codebase but do not use their ranking-based loss.
With a single Nvidia 2080 Ti, it takes around 3 minutes to finish the NeuS training and export a textured mesh. 

==> sections/legacy/5-exp-old.tex <==


\section{Experiment}

We prepare our training data using Objaverse~\cite{deitke2023objaverse} by filtering 180k objects from the full 800k dataset. Concretely, we compute the aesthetic score~\cite{ava} for each object using one rendered image and only keep objects with a score larger than 5 for training. 
%
The rendering of the training data follows the camera configuration described in \S\ref{subsec:camera}. The elevation of the reference view is randomly sampled from [-10$^\circ$, 45$^\circ$] to ensure sufficient coverage of the object. All the rendered images are with resolution 512$\times$512. 
%
At test time, we use a DDIM~\cite{song2020ddim} sampler with 75 steps to sample the multi-view images, and it takes our model 20s, 55s, 82s, and 123s to generate 8, 16, 24, and 32 images, respectively.  


% \TODO{Directly describe the running time of the image generation part here, using English instead of a table. }

% \input{tables/run_time}


% We render 32 generated images with fixed viewpoints according to the camera settings in \S\ref{subsec:camera}. For the conditional image, we render two sets: 1) we render reference images at the same azimuth as the generated images while the elevation is randomly sample from (-10, 45), 2) we render 10 conditional images for each object with random viewpoints following the procedure from zero-1-to-3~\cite{liu2023zero} with a resolution of $512\times 512$. 

Following the evaluation pipeline of previous works~\cite{liu2023zero,liu2023syncdreamer,long2023wonder3d}, we evaluate our method on the Google Scanned Objects (GSO) dataset~\cite{downs2022google} and compare it with various existing works. In the literature, single-view and sparse-view object modeling methods are mostly separate, so we divide our evaluation into two parts: \S\ref{subsec:exp-single} is for single-view object modeling, where we borrow the test settings from SyncDreamer~\cite{liu2023syncdreamer}; \S\ref{subsec:exp-sparse} is for sparse-view object modeling, where we construct a more challenging test setting and render the test images by ourselves.


% prepare two different evaluation settings with increasing difficulty. 

% We prepare two set of testing images, one is following the protocol of Syncdreamer~\cite{liu2023syncdreamer}, where the conditional image is always at the elevation of 30. The other, in contrast, is a more difficult testing set where the first conditional images is randomly sampled from the elevation from -10 to 45.

\CJC{TODO: Edit the experiment section: (1) reduce the description of the single-view baselines, because almost all are copied from SyncDreamer; (2). Make the running-time table embedded; (3). Re-arrange the layout of the figures; (4). Add more descriptions for the sparse-view experiments.}

\input{sections/5.1-single-view-exp}

\input{sections/5.2-sparse-view-exp}





==> sections/legacy/5.1-single-view-old.tex <==
\subsection{Single-view object modeling}
\label{subsec:exp-single}

\input{tables/single_view_syncdreamer_setting}


\mypara{Evaluation settings}
To evaluate the single-view conditioned experiments under a completely fair setting as prior works, we directly borrow the test data and evaluation scripts from SyncDreamer~\cite{liu2023syncdreamer}. Concretely, the single condition image (i.e., the reference image) has a fixed elevation of 30$^\circ$. There are 16 test images with azimuth 0$^\circ$, 22.5$^\circ$, $\dots$, 337.5$^\circ$ with respect to the reference image, all with a 30$^\circ$ elevation. 
The Chamfer Distances (CD) and volume IoU between the ground-truth and reconstructed shapes are reported for single-view 3D reconstruction. The PSNR, SSIM~\cite{wang2004ssim}, and LPIPS~\cite{zhang2018lpips} are reported for novel view synthesis (NVS). Note that only the first 8 views in our camera configuration overlap with SyncDreamer (i.e., with azimuths 0$^\circ$, 45$^\circ$, $\dots$, 315$^\circ$, and elevation 30$^\circ$), we compute the NVS results of our method by averaging over these 8 views.


\input{figures/single_images_qualitative}

\cjc{
\mypara{Baselines}  
We choose three state-of-the-art single-view object modeling methods as our main baselines: SyncDreamer~\cite{liu2023syncdreamer}, Wonder3D~\cite{long2023wonder3d}, and Open-LRM~\cite{openlrm}. Since we directly use the test data and scripts from SyncDreamer, we also borrow the baseline results in their paper for reference purpose, which includes Zero123~\cite{liu2023zero}, Real Fusion~\cite{melas2023realfusion}, Magic123~\cite{qian2023magic123}, One-2-3-45~\cite{liu2023one}, Point-E~\cite{nichol2022point}, and ShapE~\cite{jun2023shap}. We briefly introduce the three main baselines below:

\noindent \raisebox{0.25ex}{\tiny$\bullet$} \textit{Zero 123} This method is adept at generating novel-view images of an object from various viewpoints, based on a single input image. Notably, Zero 123 can be enhanced with the SDS loss function to enable 3D reconstruction. We have utilized the Three Studio's implementation for reconstruction with Zero 123, which incorporates several optimization strategies, thereby surpassing the reconstruction quality of the original Zero 123 framework.

\noindent \raisebox{0.25ex}{\tiny$\bullet$} \textit{Real Fusion} Operating on the principles of Stable Diffusion and SDS loss, Real Fusion specializes in single-view reconstruction. Its approach is fundamentally grounded in a deep understanding of image-based modeling.

\noindent \raisebox{0.25ex}{\tiny$\bullet$} \textit{Magic 123} This technique synergizes the capabilities of Zero 123 and Real Fusion. By amalgamating these methods, Magic 123 substantially elevates the quality of reconstruction, leveraging the strengths of both parent methods.

\noindent \raisebox{0.25ex}{\tiny$\bullet$}  \textit{One-2-3-45} This approach directly regresses Signed Distance Functions (SDFs) from the output images generated by Zero 123. For our experiments, we utilized the results produced by the official Hugging Face online demo [18] to assess its efficacy.

\noindent \raisebox{0.25ex}{\tiny$\bullet$} \textit{Point-E and ShapE} Both of these methods are advanced 3D generative models, trained on a substantial internal OpenAI 3D dataset. They are capable of transforming a single-view image into either a point cloud (Point-E) or a shape encoded in a Multilayer Perceptron (MLP) (ShapE). For Point-E, in particular, we transformed the generated point clouds into SDFs for shape reconstruction using the official models.


\noindent \raisebox{0.25ex}{\tiny$\bullet$} \textit{Syncdreamer} This method generates 16 images from fixed viewpoints given a single image input. However, it requires users to provide elevation information of the conditional image, which can be a limiting factor in some applications.

\noindent \raisebox{0.25ex}{\tiny$\bullet$} \textit{Wonder3D} Wonder3D also leverages 3D self attention to ensure geometry consistency among different views. Differently, the condition image is selected as the canonical view.  




\input{figures/single_mesh_qualitative}



\mypara{3D reconstruction} In Table~\ref{tab:single-view-sync} and Figure~\ref{fig:single-images-qualitative}, we present quantitative and qualitative results. Point-E and Shap-E often produce incomplete meshes. When directly distilling from Zero123, the shapes generated are roughly aligned with the input image, but they suffer from rough surfaces and lack consistency in the finer details of the input images. Magic123 yields smoother meshes; however, it heavily depends on the estimated depth values from the input view, which can lead to inaccuracies if the depth estimator is not robust. One-2-3-45 creates meshes based on the multiview-inconsistent outputs from Zero123. This approach captures the general geometry but tends to lose fine details. For Syncdreamer, it does not always generate plausible images because it introduces new parameters and they are trained from scratch using the obverse dataset. For wonder3D, it only generates 6 views and thus loses details. By contrast, our method outperforms others, achieving superior reconstruction quality with smooth surfaces and intricate geometrical details.

\mypara{Novel-view synthesis} In Table~\ref{tab:single-view-sync} and Figure~\ref{fig:single-images-qualitative}, we present both quantitative and qualitative evaluations of our novel view synthesis technique using the GSO dataset. Our method achieves superior Peak Signal-to-Noise Ratio (PSNR) compared to existing techniques such as SyncDreamer and Zero123. As illustrated in Figure~\ref{fig:single-images-qualitative}, the images generated by our approach demonstrate enhanced detail, attributable to high-resolution generation.



}

==> sections/legacy/vae_ft.tex <==
Before training the multi-view diffusion model, we fine-tune the VAE for the following two purposes:
\begin{enumerate}
[label={ {(\arabic*)}},leftmargin=*,topsep=0.5ex,itemsep=-0.5ex,partopsep=0.75ex,parsep=0.75ex,partopsep=0pt,wide, labelwidth=!,labelindent=0pt]
\item {\bf Simultaneously modeling of foreground mask.} When exporting the mesh from generated multi-view images, recent methods (e.g., SyncDreamer~\cite{liu2023syncdreamer} and Wonder3D~\cite{long2023wonder3d}) rely on an external segmentation model to produce accurate foreground masks, and the mask quality is vital for reconstruction quality. However, the mask information could have been captured by the rich LDM latents~\cite{wu2023datasetdm}, and simultaneous modeling of the image and the foreground mask is possible. We remove this external dependency by adding an extra input and output channel to the original VAE from the pre-trained LDM. 
\item {\bf Reducing compression rate for multi-view consistency.} VAE encoding is a lossy process and leads to inconsistencies among the multi-view latents, and the issue becomes more serious when the number of conditional and generated images increases. Therefore, we fine-tune the VAE to increase the PSNR of the reconstructed images.
\end{enumerate}

% \input{tables/vae_results}

% In summary, we fine-tune the VAE to enable simultaneous modeling of foreground mask and reduce the compression rate, and 

\noindent
The fine-tuning is conducted with images from Objaverse. We use the original codebase of LDM~\cite{rombach2022StableDiffusion}, and binary cross entropy is the reconstruction loss for the mask channel. We convert the fine-tuned VAE checkpoint to Diffusers using its official conversion script. Please check the \supp~for complete details. We denote the fine-tuned mask-aware VAE with M-VAE.

==> tables/ablation_view_num.tex <==
\begin{figure}[h]
  \begin{minipage}[b]{0.65\textwidth}
    \centering
    \includegraphics[width=\textwidth]{assets/num_view_ablation.pdf}
  \end{minipage}%
  \begin{minipage}[b]{0.34\textwidth}
    \centering
    \setlength{\tabcolsep}{3.5pt}
    \begin{tabular}{c@{\quad}cc}
       \toprule
       Views & CD $\downarrow$ & IoU$\uparrow$  \\
       \midrule
        8  & 0.0262 & 0.6020  \\
        16 & 0.0216 & 0.6532 \\
        24 & 0.0208 & 0.6657  \\
        32 & 0.0208 & 0.6689 \\
       \bottomrule
    \end{tabular}
    \vspace{0.5em}
    \end{minipage}
\caption{Ablation study on different numbers of generated views. \textbf{Left}: a qualitative comparison shows that denser views produce mesh with better quality. \textbf{Right}: quantitative results of 3D reconstruction using different numbers of generated views, evaluated on 30 GSO~\cite{downs2022gso} objects.}
% \vspace{-1em}
\label{fig:ablate-gen-views}
\end{figure}


==> tables/legacy/single_view_mesh_eval.tex <==
\begin{table}[ht]
    \centering
    \setlength{\tabcolsep}{4pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l@{\quad}cc}
       \toprule
       Method  & CD$\downarrow$ & Vol-IoU$\uparrow$ \\
       \midrule
       Realfusion~\cite{melas2023realfusion}    
       & 0.0819  & 0.2741   \\
       Magic123~\cite{qian2023magic123}
       & 0.0516 &  0.4528 \\
       One-2-3-45~\cite{liu2023one}    
       & 0.0629 &  0.4086 \\
       Point-E~\cite{nichol2022point}    
       & 0.0426 & 0.2875 \\
       Shap-E~\cite{jun2023shap}    
       & 0.0436 &  0.3584  \\
       Zero123~\cite{liu2023zero}    
       & 0.0339 &  0.5035 \\
       SyncDreamer~\cite{liu2023syncdreamer}    
       &  {0.0261}  &  {0.5421}   \\
       Ours
       &  \textbf{0.0229}  &  \textbf{0.5871} \\
       \bottomrule
    \end{tabular}
    }
    \vspace{0.5em}
    \caption{Quantitative comparison with baseline methods, using SyncDreamer's evaluation setting. We report Chamfer Distance and Volume IoU on the GSO~\cite{downs2022gso} dataset.}
    \label{tab:single-view-recon}
\end{table}

==> tables/legacy/single_view_nvs.tex <==


\begin{table}[!htb]
\begin{minipage}{0.48\textwidth}
    \centering
    \setlength{\tabcolsep}{4pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l@{\quad}cc}
       \toprule
       Method  & CD$\downarrow$ & Vol-IoU$\uparrow$ \\
       \midrule
       Realfusion~\cite{melas2023realfusion}    
       & 0.0819  & 0.2741   \\
       Magic123~\cite{qian2023magic123}
       & 0.0516 &  0.4528 \\
       One-2-3-45~\cite{liu2023one}    
       & 0.0629 &  0.4086 \\
       Point-E~\cite{nichol2022point}    
       & 0.0426 & 0.2875 \\
       Shap-E~\cite{jun2023shap}    
       & 0.0436 &  0.3584  \\
       Zero123~\cite{liu2023zero}    
       & 0.0339 &  0.5035 \\
       SyncDreamer~\cite{liu2023syncdreamer}    
       &  {0.0261}  &  {0.5421}   \\
       Ours
       &  \textbf{0.0229}  &  \textbf{0.5871} \\
       \bottomrule
    \end{tabular}
    }
    \vspace{0.5em}
    \caption{Quantitative comparison with baseline methods, using SyncDreamer's evaluation setting. We report Chamfer Distance and Volume IoU on the GSO~\cite{downs2022gso} dataset.}
    \label{tab:single-view-recon}
\end{minipage}%
\begin{minipage}{.48\textwidth}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccc}
       \toprule
       Method  & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
       \midrule       Realfusion~\cite{melas2023realfusion}    
       & 15.26 & 0.722 & 0.283  \\
       Zero123~\cite{liu2023zero}    
       & 18.93 & 0.779 & 0.166  \\
       SyncDreamer~\cite{liu2023syncdreamer}    
       & {20.05} & {0.798} & {0.146}  \\
       Ours \\
       \bottomrule
    \end{tabular}
    }
    \vspace{0.5em}
    \caption{The quantitative comparison in novel view synthesis. We report PSNR, SSIM~\cite{wang2004image}, LPIPS~\cite{zhang2018unreasonable} and reconstructed point number by COLMAP~\cite{schoenberger2016mvs} on the GSO~\cite{downs2022google} dataset.}
    \label{tab:single_view_nvs}
\end{minipage}
\end{table}

==> tables/run_time.tex <==

\begin{table}
    \centering
    \begin{tabular}{c|cccc}
    \hline
        No. views & 8  & 16 & 24 & 32 \\
    \hline
        Time (s) & 20 & 55 & 82 & 123\\
    \hline
    \end{tabular}
    \caption{Running time under different number of generation views for single view setting.}
    \label{tab:runtime}
\end{table}

==> tables/single_view_our_setting.tex <==
\begin{table}[ht]
    \centering
    \setlength{\tabcolsep}{3.5pt}
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{l@{\quad}cc@{\quad}cccc}
       \toprule
       \multicolumn{1}{l}{Task $\rightarrow$} &
\multicolumn{2}{c}{3D reconstruction} & \multicolumn{4}{c}{Novel view synthesis} \\
        \cmidrule(r){2-3}\cmidrule(r){4-7}
       Method  & Chamfer Dist.$\downarrow$ & Vol. IoU$\uparrow$ & views$^*$ & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  \\
       \midrule
       SyncDreamer~\cite{liu2023syncdreamer}  & 0.0318 & 0.5610 & 8 & 19.46 & 0.847 & 0.188  \\
       Ours & 0.0208 & 0.6648 & 32 & 20.25 & 0.864 & 0.159  \\
       \bottomrule
    \end{tabular}
    % }
    \vspace{0.5em}
    \caption{
    Quantitative evaluations of single-view object modeling, evaluating
reconstructed meshes (left) and generated images (right) based on the GSO~\cite{downs2022gso} dataset.
%Quantitative results of single-view reconstruction, using our extended evaluation setting on the GSO~\cite{downs2022gso} dataset. 
The input is a single image at a random elevation between $[-10^\circ, 45^\circ]$. Both ground-truth and generated images are 512$\times$512, rendered from the 3D objects. $^*:$ We evaluate the novel view synthesis of SyncDreamer with the 8 overlapped viewpoints between their and our output settings.}
    \label{tab:single-view-our}
\end{table}

==> tables/sparse_view_our_setting_nvs.tex <==
\begin{table}[tbh]
\caption{
Sparse-view object modeling results, evaluating
reconstructed meshes (left) and generated images (right), based on the GSO~\cite{downs2022gso} dataset.
% novel view synthesis with sparse-view input images, 
%Both ground-truth and generated images are 512$\times$512.
}
%\vspace{-2.5em}
\label{tab:sparse-view-quantitative}
%
\begin{minipage}{0.51\textwidth}
    \centering
    \setlength{\tabcolsep}{2.5pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc@{\quad}cc}
       \toprule
       Method & Views & Chamfer Dist.$\downarrow$ & Vol. IoU$\uparrow$  \\
       \midrule
       \multirow{2}*{\shortstack[c]{Sync-\\ Dreamer}} & \multirow{2}*{1} & \multirow{2}*{0.0318} & \multirow{2}*{0.5610} \\
       \\
       \midrule
       \multirow{6}*{\shortstack[c]{NeuS\cite{wang2021neus}\\ (G.T. pose)}} & 1 & 0.0536 & 0.4400  \\
       & 2 & 0.0307 & 0.5884 \\
       & 4 & 0.0158 & 0.7323 \\
       & 6 & 0.0121 & 0.7768 \\
       & 8 & 0.0105 & 0.7982 \\
       & 10 & 0.0096 & 0.8092 \\ 
       \midrule
       \multirow{6}*{Ours} & 1 & 0.0208 & 0.6689 \\
       & 2 & 0.0158 & 0.7260 \\
       & 4 & 0.0122 & 0.7737  \\
       & 6 & 0.0109 & 0.7925  \\
       & 8 & 0.0101 & 0.8033 \\
       & 10 & 0.0101  & 0.8046    \\
       \bottomrule
    \end{tabular}
    }
%    \vspace{0.5em}
\end{minipage}
\begin{minipage}{0.48\textwidth}
    \centering
    \setlength{\tabcolsep}{2.5pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c@{\quad}c@{\quad}ccc}
       \toprule
       Method & Views & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  \\
       \midrule
       \multirow{2}*{\shortstack[c]{Sync-\\ Dreamer}} & \multirow{2}*{1} & \multirow{2}*{19.46} & \multirow{2}*{0.847} & \multirow{2}*{0.188} \\
       \\
       \midrule
       \multirow{6}*{LEAP\cite{jiang2023leap}}  & 1 & 14.66 & 0.47 &0.43\\
       & 2 &16.22 &0.59 &0.36 \\
       & 4 & 16.54&0.61&0.35 \\
       & 6 &16.65&0.62&0.34\\
       & 8 &16.79&0.63&0.34\\
       & 10 &16.84&0.64&0.34\\
       \midrule
       \multirow{6}*{Ours} & 1 & 20.25 & 0.862 & 0.157 \\
       & 2 & 21.73 & 0.872 & 0.137 \\
       & 4  & 23.44 & 0.886 & 0.117 \\
       & 6 & 24.54 & 0.894 & 0.107 \\
       & 8 & 24.92 & 0.899 & 0.102 \\
       & 10 & 25.03 & 0.899 & 0.102 \\
       
       \bottomrule
    \end{tabular}
    }
%    \vspace{0.5em}
%    \label{tab:sparse-view-nvs}
\end{minipage}
\end{table}

==> tables/vae_results.tex <==
\begin{wraptable}[10]{r}{0.3\textwidth}

\centering
\begin{tabular}{cc}
    \hline
     & PSNR \\
    \hline
    VAE & 36.6 \\
    \hline
    M-VAE & 41.2 \\
    \hline
\end{tabular}
\caption{PSNR after we finetune the VAE on objaverse.}
\label{tab:mask-vae}

\end{wraptable}
